New Hubble Space Telescope Observations of Heavy Elements in Four Metal-Poor Stars

Elements heavier than the iron group are found in nearly all halo stars. A substantial number of these elements, key to understanding neutron-capture nucleosynthesis mechanisms, can only be detected in the near-ultraviolet. We report the results of an observing campaign using the Space Telescope Imaging Spectrograph on board the Hubble Space Telescope to study the detailed heavy element abundance patterns in four metal-poor stars. We derive abundances or upper limits from 27 absorption lines of 15 elements produced by neutron-capture reactions, including seven elements (germanium, cadmium, tellurium, lutetium, osmium, platinum, and gold) that can only be detected in the near-ultraviolet. We also examine 202 heavy element absorption lines in ground-based optical spectra obtained with the Magellan Inamori Kyocera Echelle Spectrograph on the Magellan-Clay Telescope at Las Campanas Observatory and the High Resolution Echelle Spectrometer on the Keck I Telescope on Mauna Kea. We have detected up to 34 elements heavier than zinc. The bulk of the heavy elements in these four stars are produced by r-process nucleosynthesis. These observations affirm earlier results suggesting that the tellurium found in metal-poor halo stars with moderate amounts of r-process material scales with the rare earth and third r-process peak elements. Cadmium often follows the abundances of the neighboring elements palladium and silver. We identify several sources of systematic uncertainty that must be considered when comparing these abundances with theoretical predictions. We also present new isotope shift and hyperfine structure component patterns for Lu II and Pb I lines of astrophysical interest.

==> tab3.tex <==

\begin{deluxetable}{ccccccccc}
\tablecaption{Atomic Data and Line-by-line Abundances
\label{atomictab}}
\tablewidth{0pt}
\tabletypesize{\scriptsize}
%\tabletypesize{\tiny}
%\rotate
\tablehead{
\colhead{Species} &
\colhead{$\lambda$} &
\colhead{E.P.} &
\colhead{$\log(gf)$} &
\colhead{Ref.} &
\colhead{$\log \epsilon$} &
\colhead{$\log \epsilon$} &
\colhead{$\log \epsilon$} &
\colhead{$\log \epsilon$} \\
\colhead{} &
\colhead{(\AA)} &
\colhead{(eV)} &
\colhead{} &
\colhead{} &
\colhead{HD~108317} &
\colhead{HD~122563} &
\colhead{HD~126238} &
\colhead{HD~128279} 
}
\startdata
Cu~\textsc{i}   & 3247.54  &  0.00  &  $-$0.06  &   1  &   $+$0.67   &   \nodata  &   \nodata  &   $+$0.85  \\
Cu~\textsc{i}   & 3273.96  &  0.00  &  $-$0.36  &   1  &   $+$0.73   &   $+$0.10  &   $+$1.53  &   $+$0.73  \\
Cu~\textsc{i}   & 5105.54  &  1.39  &  $-$1.50  &   2  &  $<+$1.38   &  $<+$0.48  &   $+$1.21  &  $<+$1.08  \\
Zn~\textsc{i}   & 3075.90  &  0.00  &  $-$3.85  &   3  &   $+$2.19   &   $+$1.76  &   $+$2.76  &   $+$2.23  \\
Zn~\textsc{i}   & 4680.14  &  4.01  &  $-$0.85  &   3  &  $<+$2.68   &   $+$2.07  &   $+$2.64  &   \nodata  \\
Zn~\textsc{i}   & 4722.16  &  4.03  &  $-$0.37  &   3  &   $+$2.29   &   $+$1.94  &   $+$2.59  &   $+$2.14  \\
Zn~\textsc{i}   & 4810.54  &  4.08  &  $-$0.15  &   3  &   $+$2.23   &   $+$2.00  &   $+$2.62  &   $+$2.17  \\
Ge~\textsc{i}   & 2651.17  &  0.17  &  $+$0.02  &   4  &   $+$0.27   &   $-$0.73  &   \nodata  &   $+$0.25  \\
Ge~\textsc{i}   & 2691.34  &  0.07  &  $-$0.70  &   4  &   $+$0.07   &   $-$1.05  &   $+$0.37: &   $-$0.22  \\
Ge~\textsc{i}   & 3039.07  &  0.88  &  $+$0.07  &   4  &   $+$0.16   &   $-$0.87  &   $+$0.73  &   $-$0.13  \\
Rb~\textsc{i}   & 7800.27  &  0.00  &  $+$0.14  &   4  &  $<+$1.40   &  $<+$1.20  &  $<+$1.70  &  $<+$1.60  \\
Sr~\textsc{i}   & 4607.33  &  0.00  &  $+$0.28  &   5  &   \nodata   &   $-$0.62  &   $+$0.48  &   \nodata  \\
Sr~\textsc{ii}  & 4077.71  &  0.00  &  $+$0.15  &   4  &   $+$0.55   &   $+$0.02  &   \nodata  &   $-$0.14  \\
Sr~\textsc{ii}  & 4161.79  &  2.94  &  $-$0.47  &   4  &   \nodata   &   $+$0.02  &   $+$0.98  &   \nodata  \\
Sr~\textsc{ii}  & 4215.52  &  0.00  &  $-$0.17  &   4  &   $+$0.41   &   $-$0.09  &   \nodata  &   $-$0.22  \\
Y~\textsc{ii}   & 3549.00  &  0.13  &  $-$0.29  &   6  &   $-$0.22   &   $-$0.70  &   $-$0.02  &   $-$0.70  \\
Y~\textsc{ii}   & 3584.51  &  0.10  &  $-$0.42  &   6  &   $-$0.28   &   \nodata  &   $+$0.01  &   \nodata  \\
Y~\textsc{ii}   & 3600.73  &  0.18  &  $+$0.34  &   6  &   $-$0.38   &   $-$0.92  &   $-$0.06  &   $-$0.86  \\
Y~\textsc{ii}   & 3601.92  &  0.10  &  $-$0.15  &   6  &   $-$0.38   &   \nodata  &   \nodata  &   $-$0.80  \\
Y~\textsc{ii}   & 3611.04  &  0.13  &  $+$0.05  &   6  &   $-$0.30   &   $-$0.84  &   $+$0.05  &   $-$0.78  \\
Y~\textsc{ii}   & 3774.33  &  0.13  &  $+$0.29  &   6  &   \nodata   &   $-$0.91  &   \nodata  &   $-$0.90  \\
Y~\textsc{ii}   & 4398.01  &  0.13  &  $-$0.75  &   6  &   \nodata   &   $-$1.15  &   \nodata  &   \nodata  \\
Y~\textsc{ii}   & 4883.68  &  1.08  &  $+$0.19  &   6  &   $-$0.48   &   $-$0.98  &   $-$0.18  &   $-$1.05  \\
Y~\textsc{ii}   & 4900.12  &  1.03  &  $+$0.03  &   6  &   $-$0.51   &   $-$1.01  &   \nodata  &   \nodata  \\
Y~\textsc{ii}   & 5087.42  &  1.08  &  $-$0.16  &   6  &   $-$0.46   &   $-$0.84  &   $-$0.16  &   $-$1.03  \\
Y~\textsc{ii}   & 5200.41  &  0.99  &  $-$0.47  &   6  &   $-$0.55   &   $-$1.08  &   $-$0.22  &   \nodata  \\
Y~\textsc{ii}   & 5205.72  &  1.03  &  $-$0.28  &   6  &   $-$0.48   &   $-$0.98  &   $-$0.18  &   \nodata  \\
Zr~\textsc{ii}  & 2567.64  &  0.00  &  $-$0.17  &   7  &   $+$0.17   &   \nodata  &   $+$0.17  &   $-$0.24  \\
Zr~\textsc{ii}  & 2699.60  &  0.04  &  $-$0.66  &   8  &   $+$0.26   &   \nodata  &   $+$0.80  &   $+$0.06  \\
Zr~\textsc{ii}  & 2700.13  &  0.09  &  $-$0.08  &   7  &   $+$0.14   &   $-$0.68  &   $+$0.44  &   $-$0.21  \\
Zr~\textsc{ii}  & 2732.72  &  0.09  &  $-$0.49  &   7  &   $+$0.62   &   \nodata  &   \nodata  &   $+$0.21  \\
Zr~\textsc{ii}  & 2758.81  &  0.00  &  $-$0.56  &   7  &   $+$0.29   &   $-$0.35  &   \nodata  &   $-$0.03  \\
Zr~\textsc{ii}  & 2915.99  &  0.47  &  $-$0.50  &   7  &   $+$0.38   &   $-$0.26  &   $+$0.71  &   $+$0.03  \\
Zr~\textsc{ii}  & 3054.84  &  1.01  &  $+$0.08  &   8  &   $+$0.38   &   $-$0.20: &   $+$1.01: &   $+$0.21  \\
Zr~\textsc{ii}  & 3095.07  &  0.04  &  $-$0.84  &   7  &   $+$0.44   &   $-$0.35  &   $+$0.77  &   $+$0.03  \\
Zr~\textsc{ii}  & 3125.92  &  0.00  &  $-$0.70  &   7  &   $+$0.53   &   $-$0.22  &   \nodata  &   \nodata  \\
Zr~\textsc{ii}  & 3129.76  &  0.04  &  $-$0.54  &   7  &   $+$0.47   &   \nodata  &   \nodata  &   \nodata  \\
Zr~\textsc{ii}  & 3273.05  &  0.16  &  $+$0.30  &   7  &   $+$0.65   &   $-$0.25  &   $+$0.82  &   $-$0.04  \\
Zr~\textsc{ii}  & 3279.26  &  0.09  &  $+$0.12  &   7  &   $+$0.35:  &   \nodata  &   \nodata  &   $-$0.10  \\
Zr~\textsc{ii}  & 3284.71  &  0.00  &  $-$0.37  &   7  &   $+$0.50   &   $-$0.16  &   $+$0.79  &   $+$0.02  \\
Zr~\textsc{ii}  & 3305.15  &  0.04  &  $-$0.65  &   7  &   $+$0.56   &   \nodata  &   \nodata  &   \nodata  \\
Zr~\textsc{ii}  & 3334.62  &  0.56  &  $-$0.69  &   7  &   $+$0.44   &   $-$0.04  &   \nodata  &   \nodata  \\
Zr~\textsc{ii}  & 3344.79  &  1.01  &  $-$0.35  &   7  &   $+$0.44   &   \nodata  &   \nodata  &   \nodata  \\
Zr~\textsc{ii}  & 3356.09  &  0.09  &  $-$0.39  &   8  &   $+$0.35   &   \nodata  &   \nodata  &   $-$0.04  \\
Zr~\textsc{ii}  & 3357.26  &  0.00  &  $-$0.66  &   7  &   $+$0.38   &   \nodata  &   \nodata  &   \nodata  \\
Zr~\textsc{ii}  & 3403.68  &  1.00  &  $-$0.60  &   7  &   $+$0.47   &   \nodata  &   $+$0.82  &   \nodata  \\
Zr~\textsc{ii}  & 3404.83  &  0.36  &  $-$0.49  &   7  &   $+$0.50   &   \nodata  &   \nodata  &   $+$0.11  \\
Zr~\textsc{ii}  & 3408.08  &  0.97  &  $-$0.66  &   7  &   $+$0.53   &   \nodata  &   $+$0.76  &   \nodata  \\
Zr~\textsc{ii}  & 3410.24  &  0.41  &  $-$0.31  &   7  &   $+$0.50   &   \nodata  &   \nodata  &   \nodata  \\
Zr~\textsc{ii}  & 3430.53  &  0.47  &  $-$0.16  &   7  &   $+$0.59   &   \nodata  &   $+$0.64  &   \nodata  \\
Zr~\textsc{ii}  & 3457.56  &  0.56  &  $-$0.47  &   8  &   $+$0.44   &   \nodata  &   \nodata  &   \nodata  \\
Zr~\textsc{ii}  & 3458.93  &  0.96  &  $-$0.48  &   7  &   \nodata   &   \nodata  &   $+$0.61  &   \nodata  \\
Zr~\textsc{ii}  & 3479.02  &  0.53  &  $-$0.67  &   7  &   $+$0.38   &   $-$0.16  &   $+$0.67  &   $-$0.01  \\
Zr~\textsc{ii}  & 3479.39  &  0.71  &  $+$0.18  &   7  &   $+$0.38   &   $-$0.19  &   $+$0.61  &   $+$0.02  \\
Zr~\textsc{ii}  & 3496.20  &  0.04  &  $+$0.26  &   7  &   $+$0.35   &   \nodata  &   \nodata  &   $-$0.19  \\
Zr~\textsc{ii}  & 3505.67  &  0.16  &  $-$0.39  &   7  &   $+$0.44   &   $-$0.22  &   $+$0.79  &   $+$0.02  \\
Zr~\textsc{ii}  & 3506.05  &  1.24  &  $-$0.68  &   8  &   \nodata   &   \nodata  &   $+$0.82  &   \nodata  \\
Zr~\textsc{ii}  & 3525.81  &  0.36  &  $-$0.96  &   7  &   \nodata   &   $-$0.04  &   \nodata  &   \nodata  \\
Zr~\textsc{ii}  & 3549.51  &  1.24  &  $-$0.72  &   7  &   \nodata   &   \nodata  &   $+$0.91  &   \nodata  \\
Zr~\textsc{ii}  & 3551.95  &  0.09  &  $-$0.36  &   7  &   \nodata   &   $-$0.16  &   $+$0.88  &   $+$0.11  \\
Zr~\textsc{ii}  & 3556.59  &  0.47  &  $+$0.07  &   7  &   $+$0.41   &   $-$0.13  &   \nodata  &   $+$0.05  \\
Zr~\textsc{ii}  & 3588.31  &  0.41  &  $-$1.13  &   7  &   \nodata   &   \nodata  &   \nodata  &   $+$0.14  \\
Zr~\textsc{ii}  & 3607.37  &  1.24  &  $-$0.70  &   7  &   \nodata   &   \nodata  &   $+$0.91  &   \nodata  \\
Zr~\textsc{ii}  & 3751.59  &  0.97  &  $+$0.00  &   7  &   $+$0.47   &   $-$0.13  &   \nodata  &   $-$0.03  \\
Zr~\textsc{ii}  & 3766.82  &  0.41  &  $-$0.83  &   7  &   $+$0.44   &   $-$0.04  &   \nodata  &   $+$0.03  \\
Zr~\textsc{ii}  & 3836.76  &  0.56  &  $-$0.12  &   7  &   $+$0.41   &   $-$0.16  &   $+$0.58  &   $+$0.03  \\
Zr~\textsc{ii}  & 3998.96  &  0.56  &  $-$0.52  &   7  &   $+$0.47   &   $+$0.02  &   $+$0.73  &   $+$0.06  \\
Zr~\textsc{ii}  & 4048.67  &  0.80  &  $-$0.53  &   7  &   $+$0.39   &   $-$0.29  &   \nodata  &   \nodata  \\
Zr~\textsc{ii}  & 4050.32  &  0.71  &  $-$1.06  &   7  &   $+$0.45   &   $-$0.11  &   $+$0.79  &   $-$0.09  \\
Zr~\textsc{ii}  & 4149.20  &  0.80  &  $-$0.04  &   7  &   $+$0.57   &   $-$0.20  &   $+$0.70  &   \nodata  \\
Zr~\textsc{ii}  & 4156.27  &  0.71  &  $-$0.78  &   7  &   $+$0.54   &   $-$0.11  &   \nodata  &   \nodata  \\
Zr~\textsc{ii}  & 4161.20  &  0.71  &  $-$0.59  &   7  &   $+$0.54   &   $-$0.14  &   \nodata  &   $+$0.00  \\
Zr~\textsc{ii}  & 4208.98  &  0.71  &  $-$0.51  &   7  &   $+$0.45   &   $-$0.11  &   $+$0.76  &   $-$0.03  \\
Zr~\textsc{ii}  & 4613.95  &  0.97  &  $-$1.54  &   7  &   \nodata   &   $-$0.10  &   $+$0.85  &   \nodata  \\
%Nb~\textsc{ii}  & 2876.96  &  0.44  &  $-$0.49  &   9  &   \nodata   &   \nodata  &   $-$0.20: &   \nodata  \\  %
Nb~\textsc{ii}  & 2950.88  &  0.51  &  $+$0.24  &   9  &   $-$0.86   &   $-$1.65  &   $-$0.26  &   $-$0.88  \\
Nb~\textsc{ii}  & 3028.44  &  0.44  &  $-$0.20  &   9  &   $-$0.86   &   $-$1.47  &   $-$0.38  &  $<-$0.69  \\
Nb~\textsc{ii}  & 3215.59  &  0.44  &  $-$0.24  &   9  &   $-$0.86   &   $-$1.49  &   $-$0.39  &  $<-$0.51  \\
Nb~\textsc{ii}  & 3225.47  &  0.29  &  $-$0.01  &   9  &   \nodata   &   \nodata  &   $-$0.39  &  $<-$0.71  \\
Mo~\textsc{i}   & 3864.10  &  0.00  &  $-$0.01  &  10  &   $-$0.23   &   $-$1.22: &   $+$0.18  &   $-$0.67  \\
Mo~\textsc{ii}  & 2871.51  &  1.54  &  $+$0.06  &  11  &  $<+$0.24   &  $<-$0.65  &  $<+$0.43  &  $<+$0.11  \\
Ru~\textsc{i}   & 3436.74  &  0.15  &  $+$0.15  &  12  &   $-$0.06   &   \nodata  &   \nodata  &   \nodata  \\
Ru~\textsc{i}   & 3498.94  &  0.00  &  $+$0.31  &  12  &   $-$0.03   &   $-$1.14  &   \nodata  &   $-$0.63  \\
Ru~\textsc{i}   & 3742.28  &  0.34  &  $-$0.18  &  12  &   \nodata   &   \nodata  &   $+$0.11  &   \nodata  \\
Ru~\textsc{i}   & 3798.90  &  0.15  &  $-$0.04  &  12  &   \nodata   &   $-$1.11: &   $+$0.11  &   \nodata  \\
Ru~\textsc{i}   & 3799.35  &  0.00  &  $+$0.02  &  12  &   \nodata   &   $-$0.72: &   $+$0.05  &   \nodata  \\
Rh~\textsc{i}   & 3396.82  &  0.00  &  $+$0.05  &  13  &   \nodata   &   \nodata  &   $-$0.46: &   \nodata  \\
Rh~\textsc{i}   & 3434.89  &  0.00  &  $+$0.45  &  14  &   \nodata   &   \nodata  &   \nodata  &  $<-$0.61  \\
Rh~\textsc{i}   & 3692.36  &  0.00  &  $+$0.17  &  13  &   $-$0.84:  &   $-$1.73: &   $-$1.06: &   \nodata  \\
Rh~\textsc{i}   & 3700.91  &  0.19  &  $-$0.10  &  13  &   \nodata   &   \nodata  &   $-$0.43: &   \nodata  \\
Pd~\textsc{i}   & 3242.70  &  0.81  &  $+$0.07  &  15  &   \nodata   &   \nodata  &   $-$0.23  &   \nodata  \\
Pd~\textsc{i}   & 3404.58  &  0.81  &  $+$0.33  &  15  &   $-$0.70   &   $-$1.78: &   $-$0.32  &   $-$1.24: \\
Pd~\textsc{i}   & 3516.94  &  0.96  &  $-$0.21  &  15  &   $-$0.61:  &  $<-$1.23  &   $-$0.41  &   \nodata  \\
Ag~\textsc{i}   & 3280.68  &  0.00  &  $-$0.02  &  16  &   $-$1.47:  &  $<-$1.95  &   \nodata  &  $<-$1.13  \\
Ag~\textsc{i}   & 3382.89  &  0.00  &  $-$0.33  &  16  &   $-$1.26:  &  $<-$1.65  &   $-$1.03: &   \nodata  \\
Cd~\textsc{i}   & 2288.02  &  0.00  &  $+$0.15  &  17  &   $-$0.87:  &  $<-$2.85  &   \nodata  &   $-$1.38: \\
Sn~\textsc{i}   & 3801.01  &  1.07  &  $-$0.74  &   4  &  $<+$0.80   &  $<+$0.38  &   \nodata  &   \nodata  \\
Te~\textsc{i}   & 2385.79  &  0.59  &  $-$0.81  &  18  &   $+$0.02   &   \nodata  &   \nodata  &   $-$0.18  \\
Ba~\textsc{ii}  & 4130.65  &  2.72  &  $+$0.52  &  19  &   $-$0.39   &   \nodata  &   \nodata  &   \nodata  \\
Ba~\textsc{ii}  & 4554.03  &  0.00  &  $+$0.14  &  19  &   $-$0.18   &   $-$1.88  &   $-$0.06  &   $-$1.08  \\
Ba~\textsc{ii}  & 5853.67  &  0.60  &  $-$0.91  &  19  &   $-$0.36   &   $-$1.68  &   $+$0.00  &   $-$1.02  \\
Ba~\textsc{ii}  & 6141.71  &  0.70  &  $-$0.03  &  19  &   $-$0.33   &   \nodata  &   \nodata  &   $-$0.99  \\
La~\textsc{ii}  & 3794.77  &  0.24  &  $+$0.21  &  20  &   $-$1.13   &   \nodata  &   $-$0.96  &   \nodata  \\
La~\textsc{ii}  & 3949.10  &  0.40  &  $+$0.49  &  20  &   $-$1.16   &   \nodata  &   \nodata  &   \nodata  \\
La~\textsc{ii}  & 3988.51  &  0.40  &  $+$0.21  &  20  &   $-$1.10   &   $-$2.51  &   $-$0.87  &   $-$1.72  \\
La~\textsc{ii}  & 3995.74  &  0.17  &  $-$0.06  &  20  &   $-$1.07   &   $-$2.27  &   $-$0.84  &   $-$1.63  \\
La~\textsc{ii}  & 4086.71  &  0.00  &  $-$0.07  &  20  &   $-$1.15   &   $-$2.61  &   $-$0.96  &   $-$1.51  \\
La~\textsc{ii}  & 4123.22  &  0.32  &  $+$0.13  &  20  &   $-$1.12   &   \nodata  &   \nodata  &   $-$1.72  \\
La~\textsc{ii}  & 4322.50  &  0.17  &  $-$0.93  &  20  &   \nodata   &   \nodata  &   $-$0.90  &   \nodata  \\
La~\textsc{ii}  & 4333.75  &  0.17  &  $-$0.06  &  20  &   $-$1.12   &   \nodata  &   \nodata  &   \nodata  \\
La~\textsc{ii}  & 4662.50  &  0.00  &  $-$1.24  &  20  &   \nodata   &   \nodata  &   $-$0.87  &   \nodata  \\
La~\textsc{ii}  & 4920.98  &  0.13  &  $-$0.58  &  20  &   \nodata   &   \nodata  &   $-$0.90  &   \nodata  \\
La~\textsc{ii}  & 4921.78  &  0.24  &  $-$0.45  &  20  &   \nodata   &   \nodata  &   $-$0.87  &   \nodata  \\
La~\textsc{ii}  & 5114.56  &  0.23  &  $-$1.03  &  20  &   \nodata   &   \nodata  &   $-$0.93  &   \nodata  \\
Ce~\textsc{ii}  & 3999.24  &  0.30  &  $+$0.06  &  21  &   $-$0.68   &   $-$1.91: &   $-$0.45  &   \nodata  \\
Ce~\textsc{ii}  & 4042.58  &  0.49  &  $+$0.00  &  21  &   $-$0.76   &   \nodata  &   $-$0.54  &   \nodata  \\
Ce~\textsc{ii}  & 4053.50  &  0.00  &  $-$0.61  &  21  &   $-$0.64   &   \nodata  &   $-$0.51  &   \nodata  \\
Ce~\textsc{ii}  & 4073.47  &  0.48  &  $+$0.21  &  21  &   $-$0.70   &   $-$1.98: &   \nodata  &   $-$1.12  \\
Ce~\textsc{ii}  & 4083.22  &  0.70  &  $+$0.27  &  21  &   $-$0.64   &   \nodata  &   $-$0.42  &   \nodata  \\
Ce~\textsc{ii}  & 4118.14  &  0.70  &  $+$0.13  &  21  &   $-$0.67   &   \nodata  &   $-$0.51  &   \nodata  \\
Ce~\textsc{ii}  & 4120.83  &  0.32  &  $-$0.37  &  21  &   $-$0.61   &   \nodata  &   $-$0.39  &   \nodata  \\
Ce~\textsc{ii}  & 4127.36  &  0.68  &  $+$0.31  &  21  &   $-$0.73   &   \nodata  &   $-$0.48  &   \nodata  \\
Ce~\textsc{ii}  & 4137.64  &  0.52  &  $+$0.40  &  21  &   $-$0.70   &   $-$1.89  &   $-$0.45  &   $-$1.15  \\
Ce~\textsc{ii}  & 4222.60  &  0.12  &  $-$0.15  &  21  &   $-$0.67   &   $-$1.92  &   $-$0.48  &   $-$1.18  \\
Ce~\textsc{ii}  & 4486.91  &  0.30  &  $-$0.18  &  21  &   \nodata   &   \nodata  &   $-$0.63  &   \nodata  \\
Ce~\textsc{ii}  & 4562.36  &  0.48  &  $+$0.21  &  21  &   $-$0.66   &   $-$1.94  &   $-$0.48  &   \nodata  \\
Ce~\textsc{ii}  & 4572.28  &  0.68  &  $+$0.22  &  21  &   \nodata   &   \nodata  &   $-$0.51  &   \nodata  \\
Ce~\textsc{ii}  & 4628.16  &  0.52  &  $+$0.14  &  21  &   \nodata   &   $-$2.03  &   $-$0.54  &   \nodata  \\
Pr~\textsc{ii}  & 4062.80  &  0.42  &  $+$0.33  &  22  &   \nodata   &   \nodata  &   $-$1.07  &   \nodata  \\
Pr~\textsc{ii}  & 4179.40  &  0.20  &  $+$0.46  &  22  &   $-$0.99:  &   \nodata  &   \nodata  &   \nodata  \\
Pr~\textsc{ii}  & 4189.49  &  0.37  &  $+$0.43  &  22  &   \nodata   &  $<-$2.15  &   \nodata  &   \nodata  \\
Pr~\textsc{ii}  & 4429.13\tablenotemark{a}  &  0.00  &  $-$0.49  &  22  &   $-$0.80:  &   \nodata  &   \nodata  &   \nodata  \\
%Pr~\textsc{ii}  & 4429.26  &  0.37  &  $-$0.05  &  22  &   $-$0.80:  &   \nodata  &   \nodata  &   \nodata  \\  %
Pr~\textsc{ii}  & 5322.77  &  0.48  &  $-$0.12  &  22  &   \nodata   &   \nodata  &   $-$1.10  &   \nodata  \\
Nd~\textsc{ii}  & 3784.24  &  0.38  &  $+$0.15  &  23  &   $-$0.72   &   $-$2.13  &   $-$0.49  &   $-$1.28  \\
Nd~\textsc{ii}  & 3810.48  &  0.74  &  $-$0.14  &  23  &   \nodata   &   \nodata  &   $-$0.31  &   \nodata  \\
Nd~\textsc{ii}  & 3826.41  &  0.06  &  $-$0.41  &  23  &   $-$0.51   &   \nodata  &   $-$0.46  &   \nodata  \\
Nd~\textsc{ii}  & 3838.98  &  0.00  &  $-$0.24  &  23  &   $-$0.78   &   \nodata  &   \nodata  &   \nodata  \\
Nd~\textsc{ii}  & 4004.00  &  0.06  &  $-$0.57  &  23  &   $-$0.74   &   \nodata  &   $-$0.55  &   \nodata  \\
Nd~\textsc{ii}  & 4012.70  &  0.00  &  $-$0.60  &  23  &   \nodata   &   \nodata  &   $-$0.46  &   \nodata  \\
Nd~\textsc{ii}  & 4018.82  &  0.06  &  $-$0.85  &  23  &   \nodata   &   \nodata  &   $-$0.64  &   \nodata  \\
Nd~\textsc{ii}  & 4021.33  &  0.32  &  $-$0.10  &  23  &   $-$0.77   &   \nodata  &   $-$0.67  &   \nodata  \\
Nd~\textsc{ii}  & 4023.00  &  0.56  &  $+$0.04  &  23  &   \nodata   &   \nodata  &   $-$0.55  &   \nodata  \\
Nd~\textsc{ii}  & 4051.14  &  0.38  &  $-$0.30  &  23  &   $-$0.74   &   \nodata  &   \nodata  &   \nodata  \\
Nd~\textsc{ii}  & 4059.95  &  0.20  &  $-$0.52  &  23  &   $-$0.68   &   \nodata  &   $-$0.58  &   \nodata  \\
Nd~\textsc{ii}  & 4069.26  &  0.06  &  $-$0.57  &  23  &   $-$0.68   &   \nodata  &   $-$0.46  &   \nodata  \\
Nd~\textsc{ii}  & 4109.45  &  0.32  &  $+$0.35  &  23  &   $-$0.65   &   $-$1.96  &   $-$0.37  &   $-$1.19  \\
Nd~\textsc{ii}  & 4133.35  &  0.32  &  $-$0.49  &  23  &   \nodata   &   \nodata  &   $-$0.46  &   \nodata  \\
Nd~\textsc{ii}  & 4232.37  &  0.06  &  $-$0.47  &  23  &   $-$0.71   &   \nodata  &   $-$0.58  &   $-$1.22  \\
Nd~\textsc{ii}  & 4446.38  &  0.20  &  $-$0.35  &  23  &   $-$0.76   &   $-$2.10  &   $-$0.58  &   $-$1.24  \\
Nd~\textsc{ii}  & 4645.76  &  0.56  &  $-$0.76  &  23  &   \nodata   &   \nodata  &   $-$0.37  &   \nodata  \\
Nd~\textsc{ii}  & 4706.54  &  0.00  &  $-$0.71  &  23  &   $-$0.76   &   \nodata  &   $-$0.34  &   \nodata  \\
Nd~\textsc{ii}  & 4914.38  &  0.38  &  $-$0.70  &  23  &   \nodata   &   \nodata  &   $-$0.58  &   \nodata  \\
Nd~\textsc{ii}  & 5092.79  &  0.38  &  $-$0.61  &  23  &   \nodata   &   \nodata  &   $-$0.61  &   \nodata  \\
Nd~\textsc{ii}  & 5234.19  &  0.55  &  $-$0.51  &  23  &   \nodata   &   \nodata  &   $-$0.55  &   \nodata  \\
Nd~\textsc{ii}  & 5249.58  &  0.98  &  $+$0.20  &  23  &   \nodata   &   \nodata  &   $-$0.58  &   \nodata  \\
Nd~\textsc{ii}  & 5255.51  &  0.20  &  $-$0.67  &  23  &   \nodata   &   \nodata  &   $-$0.52  &   \nodata  \\
Nd~\textsc{ii}  & 5293.16  &  0.82  &  $+$0.10  &  23  &   \nodata   &   \nodata  &   $-$0.61  &   \nodata  \\
Nd~\textsc{ii}  & 5319.81  &  0.55  &  $-$0.14  &  23  &   \nodata   &   \nodata  &   $-$0.58  &   \nodata  \\
Sm~\textsc{ii}  & 3568.27  &  0.48  &  $+$0.29  &  24  &   $-$0.97   &   \nodata  &   \nodata  &   $-$1.36  \\
Sm~\textsc{ii}  & 3706.75  &  0.48  &  $-$0.60  &  24  &   \nodata   &   \nodata  &   $-$0.83: &   \nodata  \\
Sm~\textsc{ii}  & 3896.97  &  0.04  &  $-$0.67  &  24  &   $-$1.06   &   \nodata  &   $-$0.86  &   \nodata  \\
Sm~\textsc{ii}  & 4318.93  &  0.28  &  $-$0.25  &  24  &   $-$1.05   &   $-$2.21  &   $-$0.86  &   \nodata  \\
Sm~\textsc{ii}  & 4424.34  &  0.48  &  $+$0.14  &  24  &   $-$1.25:  &   \nodata  &   \nodata  &   \nodata  \\
Sm~\textsc{ii}  & 4434.32  &  0.38  &  $-$0.07  &  24  &   $-$1.01:  &   $-$2.38: &   $-$0.92  &   $-$1.61  \\
Sm~\textsc{ii}  & 4467.34  &  0.66  &  $+$0.15  &  24  &   \nodata   &   $-$2.41  &   $-$0.95  &   \nodata  \\
Sm~\textsc{ii}  & 4472.41  &  0.18  &  $-$0.96  &  24  &   \nodata   &   \nodata  &   $-$1.04  &   \nodata  \\
Sm~\textsc{ii}  & 4519.63  &  0.54  &  $-$0.35  &  24  &   \nodata   &   \nodata  &   $-$1.04  &   \nodata  \\
Sm~\textsc{ii}  & 4523.91  &  0.43  &  $-$0.39  &  24  &   \nodata   &   \nodata  &   $-$1.10  &   \nodata  \\
Sm~\textsc{ii}  & 4537.94  &  0.48  &  $-$0.48  &  24  &   \nodata   &   \nodata  &   $-$0.83  &   \nodata  \\
Sm~\textsc{ii}  & 4642.23  &  0.38  &  $-$0.46  &  24  &   \nodata   &   \nodata  &   $-$0.80  &   \nodata  \\
Sm~\textsc{ii}  & 4669.64  &  0.28  &  $-$0.53  &  24  &   \nodata   &   \nodata  &   $-$0.86  &   \nodata  \\
Sm~\textsc{ii}  & 4719.84  &  0.04  &  $-$1.24  &  24  &   \nodata   &   \nodata  &   $-$1.01  &   \nodata  \\
Sm~\textsc{ii}  & 4815.80  &  0.18  &  $-$0.82  &  24  &   \nodata   &   \nodata  &   $-$0.95  &   \nodata  \\
Eu~\textsc{ii}  & 3724.93  &  0.00  &  $-$0.09  &  25  &   $-$1.32   &   \nodata  &   $-$1.12  &   \nodata  \\
Eu~\textsc{ii}  & 3819.67  &  0.00  &  $+$0.51  &  25  &   $-$1.38   &   $-$2.85  &   \nodata  &   $-$2.00  \\
Eu~\textsc{ii}  & 3907.11  &  0.21  &  $+$0.17  &  25  &   $-$1.35   &   \nodata  &   $-$1.21  &   $-$1.97  \\
Eu~\textsc{ii}  & 4129.72  &  0.00  &  $+$0.22  &  25  &   $-$1.43   &   $-$2.77  &   $-$1.24  &   $-$2.00  \\
Eu~\textsc{ii}  & 4205.04  &  0.00  &  $+$0.21  &  25  &   $-$1.34   &   $-$2.71  &   \nodata  &   $-$1.88  \\
Gd~\textsc{ii}  & 3549.36  &  0.24  &  $+$0.29  &  26  &   $-$0.80   &   \nodata  &   $-$0.69  &   \nodata  \\
Gd~\textsc{ii}  & 3557.06  &  0.60  &  $+$0.04  &  26  &   \nodata   &   \nodata  &   $-$0.47: &   \nodata  \\
Gd~\textsc{ii}  & 3712.70  &  0.38  &  $+$0.04  &  26  &   \nodata   &   \nodata  &   $-$0.72  &   \nodata  \\
Gd~\textsc{ii}  & 3768.40  &  0.08  &  $+$0.21  &  26  &   $-$0.83   &   $-$2.30  &   $-$0.66  &   \nodata  \\
Gd~\textsc{ii}  & 4037.89  &  0.56  &  $-$0.42  &  26  &   $-$0.76   &   \nodata  &   $-$0.69  &   \nodata  \\
Gd~\textsc{ii}  & 4049.85  &  0.99  &  $+$0.49  &  26  &   $-$0.92   &   \nodata  &   \nodata  &   \nodata  \\
Gd~\textsc{ii}  & 4085.56  &  0.73  &  $+$0.00  &  26  &   \nodata   &   \nodata  &   $-$0.73  &   \nodata  \\
Gd~\textsc{ii}  & 4130.37  &  0.73  &  $-$0.02  &  27  &   $-$0.64   &   \nodata  &   $-$0.51  &   \nodata  \\
Gd~\textsc{ii}  & 4215.02  &  0.43  &  $-$0.44  &  26  &   $-$0.88   &   \nodata  &   $-$0.66  &   \nodata  \\
Gd~\textsc{ii}  & 4251.73  &  0.38  &  $-$0.22  &  26  &   \nodata   &   \nodata  &   $-$0.78  &   \nodata  \\
Tb~\textsc{ii}  & 3600.41  &  0.64  &  $+$0.60  &  28  &   $-$1.29:  &   \nodata  &   \nodata  &   \nodata  \\
Tb~\textsc{ii}  & 3702.85  &  0.13  &  $+$0.44  &  28  &   \nodata   &   \nodata  &   $-$1.61  &   \nodata  \\
Dy~\textsc{ii}  & 3531.71  &  0.00  &  $+$0.77  &  29  &   $-$0.77   &   \nodata  &   $-$0.48  &   $-$1.43  \\
Dy~\textsc{ii}  & 3536.02  &  0.54  &  $+$0.53  &  29  &   $-$0.74   &   \nodata  &   $-$0.51  &   \nodata  \\
Dy~\textsc{ii}  & 3550.22  &  0.59  &  $+$0.27  &  29  &   $-$0.56   &   \nodata  &   \nodata  &   $-$1.19  \\
Dy~\textsc{ii}  & 3563.15  &  0.10  &  $-$0.36  &  29  &   $-$0.74   &   \nodata  &   $-$0.57  &   \nodata  \\
Dy~\textsc{ii}  & 3694.81  &  0.10  &  $-$0.11  &  29  &   $-$0.77   &   $-$2.39  &   $-$0.66  &   $-$1.36  \\
Dy~\textsc{ii}  & 3757.37  &  0.10  &  $-$0.17  &  29  &   $-$0.77   &   \nodata  &   \nodata  &   \nodata  \\
Dy~\textsc{ii}  & 3944.68  &  0.00  &  $+$0.11  &  29  &   $-$0.80   &   \nodata  &   \nodata  &   $-$1.39  \\
Dy~\textsc{ii}  & 3996.69  &  0.59  &  $-$0.26  &  29  &   $-$0.74   &   \nodata  &   $-$0.60  &   \nodata  \\
Dy~\textsc{ii}  & 4073.12  &  0.54  &  $-$0.32  &  29  &   $-$0.85   &   \nodata  &   $-$0.69  &   \nodata  \\
Dy~\textsc{ii}  & 4103.31  &  0.10  &  $-$0.38  &  29  &   \nodata   &   \nodata  &   $-$0.57  &   \nodata  \\
Dy~\textsc{ii}  & 4449.70  &  0.00  &  $-$1.03  &  29  &   \nodata   &   \nodata  &   $-$0.69  &   \nodata  \\
Ho~\textsc{ii}  & 3456.01  &  0.00  &  $+$0.76  &  30  &   $-$1.47:  &  $<-$2.43  &   $-$1.37: &  $<-$1.71  \\
Ho~\textsc{ii}  & 3890.97  &  0.08  &  $+$0.46  &  30  &   $-$1.51   &   \nodata  &   \nodata  &   \nodata  \\
Er~\textsc{ii}  & 3692.65  &  0.05  &  $+$0.28  &  31  &   $-$0.95   &   \nodata  &   \nodata  &   $-$1.48: \\
Er~\textsc{ii}  & 3729.52  &  0.00  &  $-$0.59  &  31  &   $-$0.89   &   \nodata  &   $-$0.78  &   \nodata  \\
Er~\textsc{ii}  & 3786.84  &  0.00  &  $-$0.52  &  31  &   $-$0.92   &   \nodata  &   \nodata  &   \nodata  \\
Er~\textsc{ii}  & 3830.48  &  0.00  &  $-$0.22  &  31  &   \nodata   &   \nodata  &   \nodata  &   $-$1.63  \\
Er~\textsc{ii}  & 3896.23  &  0.05  &  $-$0.12  &  31  &   $-$0.92   &   \nodata  &   \nodata  &   $-$1.48  \\
Er~\textsc{ii}  & 3906.31  &  0.00  &  $+$0.12  &  31  &   $-$1.01   &   \nodata  &   \nodata  &   \nodata  \\
Tm~\textsc{ii}  & 3701.36  &  0.00  &  $-$0.54  &  32  &   \nodata   &   \nodata  &   $-$1.54  &   \nodata  \\
Tm~\textsc{ii}  & 3795.76  &  0.03  &  $-$0.23  &  32  &   $-$1.86   &   \nodata  &   $-$1.66  &   \nodata  \\
Tm~\textsc{ii}  & 3848.02  &  0.00  &  $-$0.14  &  32  &   $-$1.74   &   \nodata  &   $-$1.60  &   $-$2.24  \\
Yb~\textsc{ii}  & 3694.19  &  0.00  &  $-$0.30  &  33  &   $-$1.13   &   $-$2.69  &   $-$0.93  &   $-$1.69  \\
Lu~\textsc{ii}  & 2615.41  &  0.00  &  $+$0.11  &  34  &   $-$1.64   &   $-$2.89  &   \nodata  &   $-$1.64  \\
Hf~\textsc{ii}  & 2641.41  &  1.04  &  $+$0.57  &  35  &   $-$0.87   &   $-$2.47: &   $-$0.78  &   $-$1.07  \\
Hf~\textsc{ii}  & 3176.85  &  0.61  &  $-$0.80  &  35  &   \nodata   &  $<-$1.13  &   \nodata  &   \nodata  \\
Hf~\textsc{ii}  & 4093.15  &  0.45  &  $-$1.15  &  35  &   $-$1.16:  &   \nodata  &   $-$1.09  &   \nodata  \\
Os~\textsc{i}   & 3058.66  &  0.00  &  $-$0.41  &  36  &   $-$0.50   &  $<-$1.25  &   $-$0.38: &  $<-$0.39  \\
Os~\textsc{ii}  & 2282.28  &  0.00  &  $-$0.05  &  37  &   $-$0.88   &   \nodata  &   $-$0.86: &  $<-$1.19  \\
Ir~\textsc{i}   & 2924.79  &  0.00  &  $-$0.66  &  38  &   $-$0.49:  &  $<-$1.35  &   $-$0.34: &  $<-$0.29  \\
Ir~\textsc{i}   & 3220.78  &  0.35  &  $-$0.48  &  38  &   $+$0.08   &  $<-$0.73  &   \nodata  &   \nodata  \\
Ir~\textsc{i}   & 3800.12  &  0.00  &  $-$1.43  &  38  &   $-$0.10   &  $<-$0.42  &   $-$0.26  &  $<+$0.01  \\
Pt~\textsc{i}   & 2659.45  &  0.00  &  $-$0.03  &  39  &   $-$0.49   &  $<-$2.15  &   \nodata  &  $<-$1.19  \\
Pt~\textsc{i}   & 2929.79  &  0.00  &  $-$0.70  &  39  &   $-$0.43   &  $<-$1.25  &   $-$0.34: &  $<-$0.49  \\
Au~\textsc{i}   & 2675.95  &  0.00  &  $-$0.47  &  40  &   $-$1.64:  &   \nodata  &   \nodata  &  $<-$0.49  \\
Pb~\textsc{i}   & 2833.05  &  0.00  &  $-$0.50  &  41  &  $<-$0.26   &  $<-$1.45  &  $<+$0.03  &  $<-$0.09  \\
Pb~\textsc{i}   & 3683.46  &  0.97  &  $-$0.54  &  41  &  $<+$0.35   &  $<-$0.32  &   $-$0.02  &   \nodata  \\
Pb~\textsc{i}   & 4057.81  &  1.32  &  $-$0.22  &  41  &  $<+$0.25   &  $<-$0.65  &   $+$0.31  &  $<+$0.35  \\
Bi~\textsc{i}   & 3024.64  &  1.91  &  $-$0.14  &   4  &  $<+$1.04   &  $<+$0.15  &  $<+$1.43  &  $<+$0.91  \\
Th~\textsc{ii}  & 4019.13  &  0.00  &  $-$0.23  &  42  &   $-$1.99   &   \nodata  &   \nodata  &   \nodata  \\
\enddata
\tablerefs{
(1) \citealt{fuhr09}, using hfs/IS from J.S.\ Sobeck et al.\ in prep.;
(2) \citealt{fuhr09}, using hfs/IS from \citealt{kurucz95};
(3) \citealt{roederer12b};
% (4) \citealt{biemont80};
% (4) \citealt{biemont99};
(4) \citealt{fuhr09};
(5) \citealt{migdalek87};
(6) \citealt{biemont11};
(7) \citealt{ljung06};
(8) \citealt{malcheva06};
(9) \citealt{nilsson08}, using hfs from \citealt{nilsson10} when available;
(10) \citealt{whaling88};
(11) \citealt{sikstrom01};
(12) \citealt{wickliffe94};
(13) \citealt{duquette85};
(14) \citealt{kwiatkowski82};
(15) \citealt{xu06};
(16) \citealt{hansen12} for both $\log(gf)$ and hfs/IS;
(17) \citealt{morton00};
(18) \citealt{roederer12a};
(19) \citealt{fuhr09}, using hfs/IS from \citealt{mcwilliam98};
(20) \citealt{lawler01a}, using hfs from \citealt{ivans06} when available;
(21) \citealt{lawler09};
(22) \citealt{li07}, using hfs from \citealt{sneden09};
(23) \citealt{denhartog03}, using hfs/IS from \citealt{roederer08} when available;
(24) \citealt{lawler06}, using hfs/IS from \citealt{roederer08} when available;
(25) \citealt{lawler01b}, using hfs/IS from \citealt{ivans06};
(26) \citealt{denhartog06};
(27) previously unpublished (uncertainty of 25\%);
(28) \citealt{lawler01c}, using hfs from \citealt{lawler09};
(29) \citealt{wickliffe00};
(30) \citealt{lawler04} for both $\log(gf)$ and hfs;
(31) \citealt{lawler08};
(32) \citealt{wickliffe97};
(33) \citealt{sneden09} for both $\log(gf)$ and hfs/IS;
(34) \citealt{roederer10b}, using hfs presented in Appendix~\ref{luhfs};
(35) \citealt{lawler07};
(36) \citealt{quinet06}, which is only 0.01~dex different from \citealt{cowan05} for this line;
(37) \citealt{quinet06};
(38) \citealt{xu07}, using hfs/IS from \citealt{cowan05} when available;
(39) \citealt{denhartog05} for both $\log(gf)$ and hfs/IS;
(40) \citealt{fivet06};
(41) \citealt{biemont00}, using hfs presented in Appendix~\ref{pbhfs};
(42) \citealt{nilsson02}.
}
\tablecomments{
The $\log\epsilon$ abundances listed in the Table have been corrected
according to the values given in Table~\ref{corrtab}.
 }
\tablenotetext{a}{
This feature is comprised of two Pr~\textsc{ii} transitions,
the 4429.13\,\AA\ transition with E.P.~$=$~0.00~eV and \loggf~$= -$0.49 and
the 4429.26\,\AA\ transition with E.P.~$=$~0.37~eV and \loggf~$= -$0.05.
 }
\end{deluxetable}


==> tab4.tex <==

\begin{deluxetable}{ccccc}
\tablecaption{Iron Equivalent Widths
\label{fetab}}
\tablewidth{0pt}
\tabletypesize{\scriptsize}
%\rotate
\tablehead{
\colhead{$\lambda$} &
%\colhead{Species} &
%\colhead{E.P.} &
%\colhead{$\log(gf)$} &
\colhead{HD~108317} &
\colhead{HD~122563} &
\colhead{HD~126238} &
\colhead{HD~128279} \\
\colhead{(\AA)} &
%\colhead{} &
%\colhead{(eV)} &
%\colhead{} &
\colhead{EW (m\AA)} &
\colhead{EW (m\AA)} &
\colhead{EW (m\AA)} &
\colhead{EW (m\AA)} 
}
\startdata
\multicolumn{5}{c}{Fe~\textsc{i}} \\
\hline
 3765.54 & \nodata & \nodata &   117.1 & \nodata \\
 3786.68 &    70.5 &    99.1 &   111.6 &    72.4 \\
 3805.34 & \nodata & \nodata &    92.6 & \nodata \\
 3849.97 & \nodata &   158.4 &    86.7 & \nodata \\
 3878.02 &   127.1 & \nodata & \nodata & \nodata \\
 3902.95 &   115.8 & \nodata & \nodata & \nodata \\
 3949.95 &    53.0 &    73.2 & \nodata &    57.6 \\
 4005.24 &   110.5 & \nodata & \nodata & \nodata \\
 4114.44 &    24.1 &    28.2 &    58.9 &    26.0 \\
 4132.06 &   110.1 &   138.1 & \nodata & \nodata \\
 4134.68 &    52.6 & \nodata &    83.8 &    54.5 \\
 4147.67 &    55.7 &    79.5 &    93.4 &    57.8 \\
 4154.50 &    49.3 & \nodata &    90.7 &    52.9 \\
 4156.80 &    50.9 &    54.2 & \nodata &    53.3 \\
 4157.78 &    32.2 &    36.9 &    70.7 &    38.4 \\
 4174.91 &    49.6 & \nodata & \nodata &    54.0 \\
 4175.64 &    46.8 &    52.1 &    80.9 &    48.2 \\
 4181.76 &    64.3 &    76.2 & \nodata &    68.3 \\
 4182.38 &    17.7 & \nodata &    57.4 &    20.2 \\
 4184.89 &    40.8 & \nodata &    79.0 &    41.3 \\
 4187.04 &    73.2 &    94.4 & \nodata & \nodata \\
 4187.80 &    82.3 &    96.5 & \nodata &    85.2 \\
 4191.43 &    73.6 &    85.7 & \nodata & \nodata \\
 4195.33 &    40.4 &    43.2 & \nodata &    44.2 \\
 4199.10 & \nodata & \nodata &   107.1 & \nodata \\
 4202.03 &   110.4 & \nodata & \nodata & \nodata \\
 4216.18 &    74.5 &   118.6 &   122.0 &    78.2 \\
 4217.55 &    29.0 &    31.2 &    68.2 &    33.3 \\
 4222.21 &    58.9 &    73.3 &    96.2 &    61.6 \\
 4233.60 &    70.5 &    90.9 & \nodata &    76.2 \\
 4238.81 &    41.0 & \nodata &    81.6 &    42.2 \\
 4250.12 &    79.6 & \nodata & \nodata & \nodata \\
 4250.79 &   103.4 & \nodata & \nodata & \nodata \\
 4282.40 & \nodata &    95.7 & \nodata & \nodata \\
 4375.93 &    86.7 & \nodata & \nodata & \nodata \\
 4388.41 &    16.4 &    16.9 & \nodata &    19.6 \\
 4415.12 &   110.7 &   139.7 & \nodata & \nodata \\
 4427.31 &    89.0 &   136.2 & \nodata &    92.2 \\
 4442.34 &    64.2 &    82.8 & \nodata &    66.3 \\
 4443.19 &    33.0 &    37.7 & \nodata &    34.8 \\
 4447.72 &    56.3 &    76.3 &   100.5 &    57.1 \\
 4461.65 &    79.0 & \nodata & \nodata & \nodata \\
 4466.55 &    59.8 & \nodata & \nodata &    63.9 \\
 4489.74 &    43.9 &    90.3 &    95.0 &    49.2 \\
 4494.56 &    65.1 &    88.5 &   108.7 &    67.2 \\
 4531.15 &    58.5 &    83.8 & \nodata &    59.7 \\
 4592.65 &    40.8 &    67.0 & \nodata &    46.0 \\
 4595.36 &     4.7 &     4.0 &    23.7 &     4.7 \\
 4602.94 &    55.2 &    84.8 &    96.2 &    56.5 \\
 4630.12 &     8.8 & \nodata &    42.6 &     9.6 \\
 4643.46 & \nodata & \nodata &    24.5 &     6.6 \\
 4647.43 &    20.0 &    25.0 &    60.2 &    22.5 \\
 4661.97 & \nodata & \nodata &    10.0 & \nodata \\
 4733.59 &    19.8 &    39.4 &    72.1 &    21.6 \\
 4736.77 &    36.0 &    41.4 &    78.0 &    36.2 \\
 4786.81 &    11.1 &    15.9 &    46.2 &    13.6 \\
 4789.65 &    12.2 &    12.5 & \nodata &    13.8 \\
 4800.65 & \nodata & \nodata &     9.8 & \nodata \\
 4871.32 &    66.0 &    80.8 &   110.1 &    68.5 \\
 4872.14 &    58.0 &    69.2 & \nodata &    57.7 \\
 4890.76 & \nodata &    77.2 &   109.8 & \nodata \\
 4891.49 &    79.1 & \nodata &   121.2 & \nodata \\
 4903.31 &    45.3 &    51.6 &    83.8 &    45.5 \\
 4918.99 &    66.5 &    82.8 &   108.3 &    74.3 \\
 4920.50 &    91.6 &   105.0 &   149.3 & \nodata \\
 4924.77 &    16.0 &    28.6 &    60.9 &    20.6 \\
 4938.81 &    30.3 &    42.7 &    75.3 &    34.4 \\
 4939.69 &    36.0 &    68.6 &    91.7 &    42.1 \\
 4966.09 &    21.1 &    30.2 &    64.5 &    26.2 \\
 4994.13 & \nodata &    78.0 & \nodata & \nodata \\
 5006.12 &    58.7 &    70.4 &   101.1 &    66.2 \\
 5028.13 &     8.4 & \nodata &    34.5 &     8.8 \\
 5044.21 & \nodata & \nodata &    33.7 &     7.6 \\
 5049.82 &    55.2 &    69.4 &    98.2 &    59.9 \\
 5051.63 &    62.2 & \nodata & \nodata &    66.3 \\
 5068.77 &    32.9 &    40.8 &    73.0 &    34.9 \\
 5079.22 & \nodata & \nodata & \nodata &    32.6 \\
 5079.74 & \nodata & \nodata &    90.0 &    43.7 \\
 5083.34 &    51.4 &    86.4 &    98.6 &    56.0 \\
 5123.72 & \nodata & \nodata & \nodata &    48.6 \\
 5127.36 &    36.8 &    73.1 &    89.8 &    41.5 \\
 5131.47 &    11.0 &    19.7 &    53.9 &    13.6 \\
 5141.74 &    10.9 &    20.1 &    49.2 &    13.9 \\
 5150.84 &    41.3 &    75.0 &    93.5 &    43.8 \\
 5151.91 &    27.5 &    62.4 &    86.3 &    33.7 \\
 5166.28 &    45.6 &    92.9 &    99.7 &    51.2 \\
 5171.60 &    78.0 &   109.0 &   119.7 &    85.0 \\
 5191.45 &    51.7 &    60.1 &    99.9 &    53.6 \\
 5192.34 &    58.3 &    70.6 &   106.9 &    65.2 \\
 5194.94 &    62.7 &    91.6 &   104.7 &    64.1 \\
 5198.71 &    19.8 &    35.9 &    69.2 &    26.9 \\
 5202.34 & \nodata &    59.4 & \nodata & \nodata \\
 5216.27 &    54.5 &    84.9 &   100.7 &    60.1 \\
 5217.39 &    19.1 &    23.1 &    59.4 &    22.3 \\
 5225.53 &    14.1 &    46.2 &    67.0 &    18.0 \\
 5232.94 &    77.0 &    93.2 &   121.9 &    85.6 \\
 5242.49 &    11.2 &    10.7 &    40.1 &    11.6 \\
 5266.56 &    61.1 &    72.2 &   105.0 &    65.0 \\
 5281.79 &    38.1 &    43.6 &    82.1 &    40.8 \\
 5283.62 & \nodata &    53.2 &    91.6 &    51.3 \\
 5288.53 &     3.1 & \nodata &    12.6 &     2.4 \\
 5307.36 &    16.7 &    33.2 &    64.9 &    19.9 \\
 5322.04 &     4.0 &     6.9 &    25.9 &     4.3 \\
 5332.90 &    21.5 &    45.5 &    76.1 &    25.3 \\
 5339.93 &    33.9 &    41.4 &    80.5 &    38.8 \\
 5364.87 &    22.2 &    19.3 &    50.8 &    23.4 \\
 5365.40 &     8.1 & \nodata &    34.1 &    10.5 \\
 5367.47 &    25.4 &    23.6 &    63.0 &    26.8 \\
 5369.96 &    30.7 &    28.1 &    67.4 &    32.3 \\
 5371.49 &   112.0 & \nodata &   165.9 &   114.5 \\
 5379.57 & \nodata & \nodata &    14.3 &     3.3 \\
 5383.37 &    36.2 &    36.5 & \nodata & \nodata \\
 5397.13 &    99.1 & \nodata &   147.0 &   101.2 \\
 5405.77 &   100.1 & \nodata &   148.9 &   104.4 \\
 5410.91 &    20.1 &    19.6 &    54.7 &    24.9 \\
 5415.20 &    30.9 &    36.0 &    69.9 &    37.1 \\
 5429.70 & \nodata &   146.3 &   166.9 & \nodata \\
 5434.52 &    87.4 &   125.5 &   132.2 &    92.2 \\
 5497.52 &    56.1 &    94.8 &   108.2 &    60.7 \\
 5501.47 &    48.2 &    87.2 &   100.5 &    55.7 \\
 5506.78 &    60.3 &    98.2 &   109.8 &    66.3 \\
 5586.76 &    56.0 &    61.6 &    95.2 &    59.0 \\
 5662.52 &     7.5 &     7.6 &    35.0 & \nodata \\
 5701.54 &    13.8 & \nodata & \nodata & \nodata \\
 5753.12 & \nodata &     3.7 &    23.7 & \nodata \\
 5816.37 & \nodata & \nodata &    11.6 &     2.4 \\
 6065.48 &    32.1 &    46.8 &    81.2 &    36.8 \\
 6136.61 &    47.4 &    67.4 &    94.4 &    52.2 \\
 6137.69 &    39.8 &    56.6 &    89.7 &    44.6 \\
 6151.62 & \nodata & \nodata &    17.5 & \nodata \\
 6191.56 &    48.6 & \nodata &    91.2 &    50.1 \\
 6213.43 &    13.2 &    20.9 &    51.5 &    13.7 \\
 6219.28 &    14.2 &    28.0 &    62.8 &    18.3 \\
 6230.72 &    48.8 &    69.5 &    98.2 &    55.9 \\
 6240.65 & \nodata &     3.9 &    18.2 &     3.0 \\
 6246.32 &    15.4 &    17.0 &    52.8 &    20.0 \\
 6265.13 &    13.5 & \nodata &    55.8 &    16.7 \\
 6297.79 & \nodata &    15.5 &    40.1 & \nodata \\
 6322.68 & \nodata & \nodata &    34.3 & \nodata \\
 6344.15 &     2.6 &     5.9 &    22.2 & \nodata \\
 6355.03 & \nodata &     6.6 &    25.5 &     5.7 \\
 6393.60 &    43.8 &    61.4 &    90.4 &    48.0 \\
 6421.35 &    28.8 &    45.6 &    79.7 &    33.3 \\
 6430.85 &    36.2 &    58.5 &    85.9 &    40.3 \\
 6494.98 &    60.3 &    81.0 &   106.6 &    65.4 \\
 6592.91 &    25.5 &    38.2 &    74.8 &    33.4 \\
 6593.87 &    10.4 & \nodata &    48.0 & \nodata \\
 6609.11 &     3.0 &     5.4 &    23.0 &     3.9 \\
 6677.99 &    35.8 &    50.7 &    86.7 &    40.6 \\
 6750.15 &     7.9 &    11.8 &    38.2 &     8.6 \\
\hline\hline
\multicolumn{5}{c}{Fe~\textsc{ii}} \\
\hline
 4178.86 &    39.2 &    58.2 &    71.0 &    38.9 \\
 4233.17 &    65.9 &    92.0 & \nodata &    65.1 \\
 4491.40 &    20.3 &    34.3 &    55.9 &    19.4 \\
 4515.34 &    30.6 &    44.6 &    69.0 &    27.0 \\
 4555.89 &    37.5 & \nodata & \nodata &    34.8 \\
 4576.34 &    15.3 &    22.7 &    46.7 &    13.1 \\
 4583.84 & \nodata &    84.5 &    99.0 &    59.2 \\
 4620.52 & \nodata &    12.5 &    30.0 &     6.9 \\
 5197.58 &    29.9 &    39.1 & \nodata &    26.1 \\
 5234.62 &    30.6 &    43.3 &    66.7 &    30.6 \\
 5276.00 &    41.1 &    51.9 &    80.8 &    39.1 \\
% 5325.55 &     4.2 &     8.7 &    18.7 &     4.0 \\
 5414.07 & \nodata &     3.8 &     7.3 & \nodata \\
\enddata
%\tablecomments{
%The complete version of Table~\ref{fetab} is available online only.
%A short version is shown here to demonstrate its form and content.
% }
\end{deluxetable}


==> tab9.tex <==
\begin{deluxetable}{ccccccc}
\tablecaption{Line-by-line Iron Abundances
\label{irontab}}
\tablewidth{0pt}
\tabletypesize{\scriptsize}
%\rotate
\tablehead{
\colhead{} &
\colhead{} &
\colhead{} &
\colhead{HD~108317} &
\colhead{HD~122563} &
\colhead{HD~126238} &
\colhead{HD~128279} \\
\colhead{Wavelength} &
\colhead{E.P.} &
\colhead{$\log(gf)$} &
\colhead{$\log\epsilon$} &
\colhead{$\log\epsilon$} &
\colhead{$\log\epsilon$} &
\colhead{$\log\epsilon$} \\
\colhead{(\AA)} &
\colhead{(eV)} &
\colhead{} &
\colhead{} &
\colhead{} &
\colhead{} &
\colhead{} }
\startdata
\multicolumn{7}{c}{Fe~\textsc{i}} \\
\hline
2283.30  & 0.12   &   $-$2.22  &   5.31     & \nodata  & \nodata  & 5.34    \\
2369.46  & 0.11   &   $-$2.20  &   5.02     & 4.49     & \nodata  & 4.92    \\
2371.43  & 0.09   &   $-$1.95  &   5.13     & 4.39     & \nodata  & 5.14    \\
2445.21  & 0.86   &   $-$2.02  &   4.95     & \nodata  & \nodata  & \nodata \\
2462.18  & 0.05   &   $-$1.30  &   4.99     & \nodata  & \nodata  & 5.07    \\
2476.66  & 0.99   &   $-$1.08  &   4.65     & \nodata  & \nodata  & \nodata \\
2486.69  & 0.96   &   $-$0.91  &   4.91     & 4.20     & \nodata  & 4.74    \\
2539.36  & 0.92   &   $-$1.79  &   5.24     & \nodata  & \nodata  & 5.02    \\
2644.00  & 1.01   &   $-$0.91  &   4.81     & \nodata  & 5.20     & 4.87    \\
2645.42  & 0.11   &   $-$2.75  &   4.85     & \nodata  & 5.38     & 4.84    \\
2647.56  & 0.05   &   $-$2.42  &   5.11     & \nodata  & 5.56     & 5.10    \\
2656.79  & 1.48   &   $-$1.77  &   5.06     & \nodata  & \nodata  & \nodata \\
2717.79  & 0.96   &   $-$1.97  &   4.92     & \nodata  & 5.60     & 4.72    \\
2730.98  & 1.01   &   $-$1.68  &   4.97     & \nodata  & \nodata  & 4.90    \\
2738.21  & 1.01   &   $-$2.64  &   5.00     & \nodata  & \nodata  & 5.09    \\
2754.03  & 0.99   &   $-$1.38  &   4.99     & 4.48     & \nodata  & 5.06    \\
2769.67  & 0.86   &   $-$2.13  &   5.19     & \nodata  & \nodata  & 5.21    \\
2867.31  & 1.61   &   $-$1.97  &   4.93     & 4.35     & 5.54     & 4.95    \\
2920.69  & 1.61   &   $-$1.39  &   4.93     & \nodata  & \nodata  & 4.88    \\
2929.62  & 1.61   &   $-$2.22  &   4.89     & \nodata  & 5.31     & 4.95    \\
2980.53  & 2.76   &   $-$0.81  &   5.01     & \nodata  & \nodata  & 5.10    \\
2990.39  & 2.73   &   $-$0.28  &   4.75     & 4.13     & 5.56     & 4.89    \\
2996.39  & 2.42   &   $-$0.94  &   4.77     & 4.03     & \nodata  & 4.87    \\
3003.03  & 0.96   &   $-$1.30  &   5.14     & 4.45     & 5.78     & 5.10    \\
3004.11  & 2.43   &   $-$1.38  &   4.69     & \nodata  & 5.45     & 4.88    \\
3009.57  & 0.91   &   $-$0.76  &   5.05     & 4.72     & 5.84     & 5.26    \\
3011.48  & 2.76   &   $-$0.33  &   4.79     & \nodata  & \nodata  & 4.85    \\
3014.17  & 0.96   &   $-$2.76  &   4.82     & 4.58     & \nodata  & 4.96    \\
3015.92  & 2.43   &   $-$1.11  &   5.02     & \nodata  & \nodata  & 5.26    \\
3016.18  & 0.99   &   $-$1.44  &   4.88     & \nodata  & \nodata  & \nodata \\
3039.32  & 2.43   &   $-$1.54  &   5.13     & 4.62     & \nodata  & 5.14    \\
3055.26  & 1.56   &   $-$1.18  &   5.25     & 4.92     & \nodata  & 5.36    \\
3180.22  & 2.45   &   $-$0.22  &   5.01     & 4.47     & 5.50     & 4.97    \\
3188.82  & 2.48   &   $-$0.72  &   5.01     & 4.45     & 5.62     & 5.01    \\
3207.08  & 2.40   &   $-$1.58  &   5.11     & \nodata  & \nodata  & 5.10    \\
3230.96  & 2.45   &   $-$0.54  &   4.84     & 4.28     & 5.32     & 4.96    \\
3246.48  & 2.59   &   $-$1.45  &   5.04     & 4.39     & 5.54     & 5.08    \\
3248.20  & 2.45   &   $-$0.67  &   5.00     & \nodata  & 5.35     & 5.03    \\
3253.60  & 3.25   &   $-$0.64  &   4.97     & 4.34     & 5.46     & 5.22    \\
3257.59  & 2.18   &   $-$1.15  &   4.89     & 4.38     & 5.40     & 4.96    \\
3259.99  & 2.45   &   $-$1.37  &   5.17     & \nodata  & 5.79     & 5.27    \\
3264.51  & 2.20   &   $-$1.32  &   4.86     & 4.25     & 5.47     & 4.97    \\
3265.05  & 0.09   &   $-$3.00  &   5.02     & 4.70     & 5.71     & 4.95    \\
3265.62  & 2.18   &   $-$0.61  &   4.83     & 4.09     & \nodata  & 4.89    \\
3268.23  & 2.22   &   $-$1.54  &   4.96     & 4.30     & 5.55     & 5.00    \\
3272.60  & 1.56   &   $-$3.19  &   4.98     & \nodata  & 5.60     & 5.03    \\
3280.26  & 3.30   &   $-$0.13  &   4.97     & \nodata  & \nodata  & 5.03    \\
3293.14  & 1.61   &   $-$3.12  &   5.21     & 4.52     & 5.58     & 5.18    \\
3323.74  & 2.83   &   $-$0.63  &   4.94     & 4.33     & 5.26     & 4.95    \\
3324.54  & 2.40   &   $-$1.50  &   5.06     & 4.36     & 5.57     & 5.06    \\
3325.46  & 2.45   &   $-$1.56  &   5.04     & \nodata  & 5.37     & \nodata \\
3328.87  & 3.27   &   $-$0.39  &   4.97     & \nodata  & 5.30     & 5.03    \\
3331.61  & 2.43   &   $-$1.57  &   4.91     & 4.29     & 5.38     & 5.00    \\
3335.77  & 2.85   &   $-$1.20  &   5.09     & \nodata  & 5.64     & \nodata \\
3337.66  & 2.69   &   $-$1.04  &   4.84     & \nodata  & 5.37     & 4.95    \\
3339.19  & 2.45   &   $-$1.69  &   4.82     & \nodata  & 5.29     & \nodata \\
3351.52  & 2.20   &   $-$2.10  &   5.01     & \nodata  & \nodata  & 5.13    \\
3351.74  & 2.73   &   $-$1.59  &   5.13     & \nodata  & 5.60     & 5.05    \\
3354.06  & 2.86   &   $-$1.17  &   4.88     & \nodata  & 5.52     & \nodata \\
3355.23  & 3.30   &   $-$0.40  &   4.95     & \nodata  & 5.37     & \nodata \\
3379.02  & 2.18   &   $-$1.41  &   5.01     & 4.56     & 5.52     & 5.10    \\
3380.11  & 2.76   &   $-$0.70  &   5.06     & 4.60     & \nodata  & 5.16    \\
3381.33  & 2.85   &   $-$1.86  &   4.92     & 4.57     & 5.52     & 4.96    \\
3382.40  & 2.18   &   $-$1.91  &   5.05     & \nodata  & \nodata  & \nodata \\
3383.98  & 2.18   &   $-$1.11  &   5.09     & \nodata  & \nodata  & \nodata \\
3392.30  & 2.20   &   $-$1.07  &   4.81     & 4.33     & 5.39     & 4.89    \\
3396.98  & 0.96   &   $-$2.43  &   4.95     & \nodata  & 5.61     & 4.92    \\
3397.64  & 0.99   &   $-$3.17  &   5.03     & \nodata  & \nodata  & \nodata \\
3410.90  & 0.91   &   $-$3.31  &   4.87     & 4.35     & 5.53     & 5.00    \\
3411.35  & 2.73   &   $-$1.02  &   4.91     & \nodata  & 5.37     & 4.97    \\
3418.51  & 2.22   &   $-$0.76  &   4.89     & 4.15     & 5.44     & 4.96    \\
3424.28  & 2.18   &   $-$0.70  &   4.85     & \nodata  & \nodata  & 4.95    \\
3425.01  & 3.05   &   $-$0.50  &   4.88     & \nodata  & \nodata  & \nodata \\
3428.19  & 2.20   &   $-$0.82  &   4.89     & \nodata  & \nodata  & 4.93    \\
3431.81  & 2.83   &   $-$1.16  &   4.92     & \nodata  & 5.40     & 4.97    \\
3442.36  & 2.28   &   $-$1.39  &   5.06     & 4.48     & 5.47     & 5.06    \\
3442.67  & 0.96   &   $-$2.66  &   4.95     & \nodata  & \nodata  & 5.03    \\
3445.15  & 2.20   &   $-$0.54  &   4.82     & \nodata  & 5.39     & 4.80    \\
3447.28  & 2.20   &   $-$1.02  &   4.83     & \nodata  & \nodata  & 4.85    \\
3451.91  & 2.22   &   $-$1.00  &   4.96     & 4.42     & 5.47     & 4.92    \\
3452.27  & 0.96   &   $-$1.92  &   4.94     & 4.55     & 5.45     & 4.86    \\
3463.30  & 1.48   &   $-$2.72  &   4.85     & \nodata  & 5.35     & 4.87    \\
3466.50  & 0.86   &   $-$2.70  &   4.86     & 4.39     & 5.34     & 4.85    \\
3468.84  & 2.56   &   $-$1.29  &   5.01     & 4.43     & \nodata  & 5.10    \\
3469.01  & 3.30   &   $-$0.86  &   5.08     & 4.52     & \nodata  & 5.13    \\
3469.83  & 2.61   &   $-$1.56  &   5.01     & 4.53     & 5.61     & 5.11    \\
3476.34  & 3.60   &   $-$0.46  &   4.64     & \nodata  & \nodata  & 4.73    \\
3493.69  & 2.73   &   $-$1.85  &   4.83     & \nodata  & 5.57     & \nodata \\
3500.56  & 2.59   &   $-$1.31  &   4.92     & 4.55     & 5.48     & 4.99    \\
3505.06  & 3.02   &   $-$1.01  &   4.97     & 4.45     & 5.49     & 5.03    \\
3512.23  & 2.85   &   $-$1.49  &   4.99     & 4.58     & \nodata  & 5.02    \\
3514.63  & 2.40   &   $-$2.02  &   4.95     & \nodata  & \nodata  & 5.03    \\
3516.41  & 3.02   &   $-$1.22  &   5.16     & 4.62     & 5.75     & 5.22    \\
3516.56  & 2.87   &   $-$1.20  &   4.91     & 4.39     & 5.51     & 4.97    \\
3518.87  & 2.20   &   $-$1.96  &   4.96     & 4.50     & 5.62     & 5.04    \\
3522.27  & 2.83   &   $-$0.99  &   5.01     & 4.41     & 5.51     & 5.07    \\
3522.90  & 2.88   &   $-$1.34  &   4.96     & 4.42     & \nodata  & 5.03    \\
3530.39  & 2.81   &   $-$0.95  &   4.97     & 4.45     & \nodata  & 5.04    \\
3537.49  & 2.59   &   $-$1.53  &   4.97     & 4.54     & 5.52     & 5.05    \\
3537.73  & 2.61   &   $-$1.13  &   4.95     & 4.40     & 5.47     & 5.01    \\
3537.89  & 2.83   &   $-$0.78  &   5.06     & 4.57     & 5.67     & 5.17    \\
3540.12  & 2.87   &   $-$0.80  &   4.99     & 4.47     & 5.61     & 5.10    \\
3540.71  & 0.91   &   $-$2.49  &   4.88     & 4.42     & \nodata  & 4.96    \\
3543.38  & 2.43   &   $-$2.00  &   4.96     & \nodata  & 5.54     & 5.02    \\
3543.67  & 3.41   &   $-$0.81  &   5.09     & 4.56     & \nodata  & 5.18    \\
3544.63  & 2.61   &   $-$1.82  &   5.15     & 4.58     & 5.73     & 5.21    \\
3547.19  & 3.30   &   $-$0.92  &   4.86     & \nodata  & 5.46     & 4.97    \\
3549.86  & 1.61   &   $-$2.46  &   5.03     & 4.53     & 5.65     & 5.12    \\
3552.11  & 3.07   &   $-$1.34  &   5.05     & 4.58     & 5.68     & 5.17    \\
3553.74  & 3.57   &   $+$0.27  &   4.78     & 4.30     & 5.38     & 4.84    \\
3554.50  & 2.88   &   $-$1.03  &   4.98     & 4.42     & 5.55     & 5.00    \\
3559.50  & 3.07   &   $-$0.91  &   4.97     & 4.36     & 5.52     & 5.03    \\
3567.03  & 2.88   &   $-$0.95  &   4.92     & \nodata  & 5.50     & 5.05    \\
3567.37  & 2.45   &   $-$2.09  &   5.00     & 4.40     & 5.66     & 4.99    \\
3568.43  & 2.88   &   $-$1.52  &   5.02     & 4.47     & 5.61     & 5.02    \\
3568.82  & 3.25   &   $-$0.94  &   5.07     & 4.52     & \nodata  & 5.11    \\
3568.97  & 2.69   &   $-$1.10  &   5.03     & 4.41     & \nodata  & 5.04    \\
3571.23  & 1.48   &   $-$2.52  &   5.00     & \nodata  & \nodata  & 5.02    \\
3573.39  & 3.30   &   $-$0.85  &   5.07     & 4.53     & \nodata  & 5.06    \\
3578.38  & 2.89   &   $-$1.35  &   5.06     & 4.45     & 5.55     & 5.14    \\
3586.74  & 2.81   &   $-$1.04  &   4.93     & 4.40     & 5.51     & 4.98    \\
3588.92  & 2.88   &   $-$0.90  &   4.99     & \nodata  & 5.51     & 5.07    \\
3589.45  & 2.73   &   $-$0.85  &   4.96     & 4.41     & \nodata  & 5.00    \\
3590.08  & 2.95   &   $-$1.71  &   5.00     & 4.34     & 5.56     & 4.98    \\
3595.30  & 2.88   &   $-$1.10  &   4.96     & 4.37     & 5.46     & 5.00    \\
3597.02  & 3.27   &   $-$0.98  &   4.95     & 4.38     & 5.43     & 4.97    \\
3599.63  & 3.57   &   $-$0.39  &   4.95     & 4.29     & 5.42     & \nodata \\
3608.14  & 2.85   &   $-$0.87  &   4.95     & \nodata  & 5.57     & 5.02    \\
3610.69  & 2.88   &   $-$1.21  &   4.97     & 4.53     & \nodata  & 5.06    \\
3615.19  & 3.28   &   $-$1.45  &   5.12     & 4.60     & 5.65     & 5.15    \\
3616.32  & 2.42   &   $-$2.17  &   4.98     & 4.48     & 5.66     & 5.03    \\
3620.24  & 2.85   &   $-$1.74  &   5.01     & 4.39     & 5.50     & 4.99    \\
3621.72  & 3.57   &   $-$0.72  &   5.15     & 4.61     & 5.55     & 5.14    \\
3623.45  & 2.56   &   $-$1.60  &   5.01     & 4.54     & 5.69     & 5.05    \\
3624.31  & 2.42   &   $-$2.00  &   4.86     & \nodata  & \nodata  & 4.94    \\
3625.14  & 2.83   &   $-$0.84  &   5.08     & \nodata  & 5.67     & 5.16    \\
3632.56  & 2.95   &   $-$0.99  &   4.99     & 4.44     & 5.54     & 5.04    \\
3637.25  & 2.43   &   $-$1.80  &   4.92     & 4.43     & \nodata  & 4.96    \\
3637.87  & 2.94   &   $-$0.97  &   5.00     & 4.47     & \nodata  & 5.09    \\
3690.45  & 3.11   &   $-$1.13  &   4.83     & \nodata  & \nodata  & \nodata \\
3690.73  & 3.57   &   $-$0.17  &   4.78     & \nodata  & \nodata  & \nodata \\
3693.03  & 3.02   &   $-$1.42  &   4.94     & 4.55     & \nodata  & \nodata \\
3715.91  & 2.28   &   $-$1.57  &   5.01     & 4.45     & 5.60     & 5.09    \\
3718.41  & 2.76   &   $-$1.12  &   5.00     & 4.36     & \nodata  & 4.97    \\
3725.49  & 3.05   &   $-$1.49  &   5.06     & 4.51     & 5.60     & 5.10    \\
3726.93  & 3.04   &   $-$0.32  &   4.86     & 4.31     & 5.44     & 4.92    \\
3727.09  & 2.94   &   $-$0.60  &   4.87     & 4.39     & 5.42     & 4.97    \\
3740.24  & 3.25   &   $-$0.62  &   5.04     & 4.45     & 5.57     & 5.09    \\
3742.62  & 2.94   &   $-$0.89  &   5.10     & 4.52     & \nodata  & 5.14    \\
3744.10  & 3.04   &   $-$0.70  &   4.97     & 4.37     & 5.41     & 5.04    \\
3756.07  & 2.18   &   $-$2.12  &   4.96     & 4.45     & 5.44     & 5.00    \\
3756.94  & 3.57   &   $-$0.28  &   4.92     & 4.38     & \nodata  & 4.99    \\
3760.05  & 2.40   &   $-$0.85  &   4.93     & \nodata  & 5.45     & 4.92    \\
3760.53  & 2.22   &   $-$1.23  &   4.92     & 4.31     & \nodata  & 4.92    \\
3765.54  & 3.24   &   $+$0.48  &   \nodata  & \nodata  & 5.77     & \nodata \\
3778.51  & 3.25   &   $-$0.90  &   5.05     & 4.53     & 5.57     & \nodata \\
3778.70  & 2.20   &   $-$2.01  &   4.84     & 4.31     & \nodata  & 4.94    \\
3781.19  & 2.20   &   $-$1.94  &   4.96     & 4.45     & 5.43     & 5.02    \\
3781.94  & 3.64   &   $-$1.24  &   5.04     & 4.34     & 5.58     & 5.06    \\
3782.45  & 3.00   &   $-$1.75  &   5.15     & \nodata  & 5.65     & \nodata \\
3786.68  & 1.01   &   $-$2.22  &   5.07     & 4.68     & 5.76     & 5.05    \\
3787.16  & 3.64   &   $-$0.97  &   5.06     & \nodata  & \nodata  & 5.13    \\
3805.34  & 3.30   &   $+$0.31  &   \nodata  & \nodata  & 5.48     & \nodata \\
3808.28  & 3.02   &   $-$1.94  &   5.05     & \nodata  & \nodata  & 5.06    \\
3808.73  & 2.56   &   $-$1.16  &   5.06     & 4.43     & \nodata  & 5.08    \\
3809.04  & 2.86   &   $-$1.95  &   4.99     & \nodata  & \nodata  & 4.93    \\
3810.76  & 3.30   &   $-$0.90  &   5.07     & \nodata  & \nodata  & 5.10    \\
3813.63  & 2.69   &   $-$1.39  &   4.88     & 4.44     & 5.43     & 4.92    \\
3817.64  & 3.33   &   $-$0.73  &   5.08     & \nodata  & \nodata  & \nodata \\
3845.17  & 2.42   &   $-$1.39  &   4.97     & 4.45     & 5.56     & 5.04    \\
3845.70  & 3.55   &   $-$1.04  &   4.93     & \nodata  & 5.44     & 4.95    \\
3845.98  & 3.37   &   $-$1.15  &   4.97     & 4.52     & 5.54     & 5.02    \\
3846.41  & 3.57   &   $-$0.47  &   4.98     & 4.46     & \nodata  & 5.07    \\
3849.97  & 1.01   &   $-$0.87  &   \nodata  & 4.49     & \nodata  & \nodata \\
3853.46  & 2.95   &   $-$1.94  &   4.93     & \nodata  & \nodata  & 4.95    \\
3854.37  & 3.21   &   $-$1.10  &   5.05     & \nodata  & \nodata  & 5.10    \\
3863.74  & 2.69   &   $-$1.43  &   5.01     & 4.51     & \nodata  & 5.11    \\
3867.22  & 3.02   &   $-$0.45  &   4.92     & 4.30     & 5.40     & 4.94    \\
3867.92  & 2.59   &   $-$1.85  &   4.93     & 4.43     & 5.45     & 4.98    \\
3878.02  & 0.96   &   $-$0.91  &   4.98     & \nodata  & \nodata  & \nodata \\
3902.95  & 1.56   &   $-$0.47  &   4.94     & \nodata  & \nodata  & \nodata \\
3949.95  & 2.18   &   $-$1.25  &   4.96     & 4.58     & 5.50     & 5.02    \\
4005.24  & 1.56   &   $-$0.61  &   4.92     & \nodata  & \nodata  & \nodata \\
4114.44  & 2.83   &   $-$1.30  &   5.01     & 4.42     & 5.45     & 5.04    \\
4132.06  & 1.61   &   $-$0.68  &   5.03     & 4.50     & \nodata  & \nodata \\
4134.68  & 2.83   &   $-$0.65  &   4.99     & \nodata  & 5.43     & 4.98    \\
4147.67  & 1.48   &   $-$2.10  &   4.97     & 4.44     & 5.48     & 4.96    \\
4154.50  & 2.83   &   $-$0.69  &   4.95     & \nodata  & 5.64     & 4.98    \\
4156.80  & 2.83   &   $-$0.81  &   5.11     & 4.42     & \nodata  & 5.11    \\
4157.78  & 3.42   &   $-$0.40  &   4.94     & 4.43     & 5.51     & 5.05    \\
4174.91  & 0.91   &   $-$2.97  &   5.06     & \nodata  & \nodata  & 5.11    \\
4175.64  & 2.85   &   $-$0.83  &   5.06     & 4.42     & 5.54     & 5.05    \\
4181.75  & 2.83   &   $-$0.37  &   4.98     & 4.40     & \nodata  & 5.01    \\
4182.38  & 3.02   &   $-$1.18  &   4.92     & \nodata  & 5.50     & 4.97    \\
4184.89  & 2.83   &   $-$0.87  &   4.95     & \nodata  & 5.51     & 4.93    \\
4187.04  & 2.45   &   $-$0.55  &   4.84     & 4.43     & \nodata  & \nodata \\
4187.80  & 2.43   &   $-$0.55  &   5.01     & 4.44     & \nodata  & 5.02    \\
4191.43  & 2.47   &   $-$0.67  &   5.03     & 4.43     & \nodata  & \nodata \\
4195.33  & 3.33   &   $-$0.49  &   5.10     & 4.51     & \nodata  & 5.15    \\
4199.10  & 3.05   &   $+$0.16  &   \nodata  & \nodata  & 5.48     & \nodata \\
4202.03  & 1.48   &   $-$0.71  &   4.90     & \nodata  & \nodata  & \nodata \\
4216.18  & 0.00   &   $-$3.36  &   5.05     & 4.61     & 5.65     & 5.07    \\
4217.55  & 3.43   &   $-$0.48  &   4.95     & 4.40     & 5.52     & 5.02    \\
4222.21  & 2.45   &   $-$0.97  &   4.92     & 4.37     & 5.47     & 4.93    \\
4233.60  & 2.48   &   $-$0.60  &   4.87     & 4.45     & \nodata  & 4.95    \\
4238.81  & 3.40   &   $-$0.23  &   4.92     & \nodata  & 5.55     & 4.92    \\
4250.12  & 2.47   &   $-$0.40  &   4.86     & \nodata  & \nodata  & \nodata \\
4250.79  & 1.56   &   $-$0.71  &   4.85     & \nodata  & \nodata  & \nodata \\
4282.40  & 2.18   &   $-$0.78  &   \nodata  & 4.40     & \nodata  & \nodata \\
4375.93  & 0.00   &   $-$3.03  &   4.98     & \nodata  & \nodata  & \nodata \\
4388.41  & 3.60   &   $-$0.68  &   4.99     & 4.45     & \nodata  & 5.07    \\
4415.12  & 1.61   &   $-$0.62  &   4.87     & 4.31     & \nodata  & \nodata \\
4427.31  & 0.05   &   $-$3.04  &   4.98     & 4.46     & \nodata  & 4.97    \\
4442.34  & 2.20   &   $-$1.26  &   5.03     & 4.48     & \nodata  & 5.02    \\
4443.19  & 2.86   &   $-$1.04  &   4.91     & 4.30     & \nodata  & 4.92    \\
4447.72  & 2.22   &   $-$1.34  &   4.98     & 4.48     & 5.65     & 4.95    \\
4461.65  & 0.09   &   $-$3.21  &   5.00     & \nodata  & \nodata  & \nodata \\
4466.55  & 2.83   &   $-$0.60  &   5.02     & \nodata  & \nodata  & 5.06    \\
4489.74  & 0.12   &   $-$3.97  &   4.92     & 4.56     & 5.50     & 4.98    \\
4494.56  & 2.20   &   $-$1.14  &   4.96     & 4.50     & 5.61     & 4.94    \\
4531.15  & 1.48   &   $-$2.16  &   4.96     & 4.42     & \nodata  & 4.93    \\
4592.65  & 1.56   &   $-$2.45  &   5.04     & 4.55     & \nodata  & 5.10    \\
4595.36  & 3.30   &   $-$1.76  &   5.06     & 4.39     & 5.59     & 5.05    \\
4602.94  & 1.48   &   $-$2.22  &   5.01     & 4.55     & 5.51     & 4.98    \\
4630.12  & 2.28   &   $-$2.59  &   5.07     & \nodata  & 5.62     & 5.09    \\
4643.46  & 3.65   &   $-$1.15  &   \nodata  & \nodata  & 5.40     & 4.97    \\
4647.43  & 2.95   &   $-$1.35  &   4.99     & 4.45     & 5.53     & 5.04    \\
4661.97  & 2.99   &   $-$2.50  &   \nodata  & \nodata  & 5.51     & \nodata \\
4733.59  & 1.48   &   $-$2.99  &   5.00     & 4.51     & 5.66     & 5.02    \\
4736.77  & 3.21   &   $-$0.75  &   5.04     & 4.49     & 5.61     & 5.02    \\
4786.81  & 3.02   &   $-$1.61  &   4.99     & 4.52     & 5.56     & 5.07    \\
4789.65  & 3.55   &   $-$0.96  &   4.97     & 4.41     & \nodata  & 5.02    \\
4800.65  & 4.14   &   $-$1.03  &   \nodata  & \nodata  & 5.34     & \nodata \\
4871.32  & 2.87   &   $-$0.36  &   4.86     & 4.34     & 5.49     & 4.87    \\
4872.14  & 2.88   &   $-$0.57  &   4.92     & 4.35     & \nodata  & 4.88    \\
4890.76  & 2.88   &   $-$0.39  &   \nodata  & 4.31     & 5.53     & \nodata \\
4891.49  & 2.85   &   $-$0.11  &   4.86     & \nodata  & 5.42     & \nodata \\
4903.31  & 2.88   &   $-$0.93  &   5.03     & 4.41     & 5.50     & 5.00    \\
4918.99  & 2.87   &   $-$0.34  &   4.83     & 4.32     & 5.40     & 4.94    \\
4920.50  & 2.83   &   $+$0.07  &   4.90     & 4.32     & 5.62     & \nodata \\
4924.77  & 2.28   &   $-$2.11  &   4.87     & 4.42     & 5.47     & 4.99    \\
4938.81  & 2.88   &   $-$1.08  &   4.88     & 4.41     & 5.46     & 4.94    \\
4939.69  & 0.86   &   $-$3.34  &   4.91     & 4.39     & 5.57     & 4.99    \\
4966.09  & 3.33   &   $-$0.87  &   4.94     & 4.54     & 5.55     & 5.05    \\
5006.12  & 2.83   &   $-$0.62  &   4.91     & 4.33     & 5.49     & 5.02    \\
5028.13  & 3.57   &   $-$1.12  &   4.97     & \nodata  & 5.48     & 4.97    \\
5049.82  & 2.28   &   $-$1.36  &   4.99     & 4.35     & 5.54     & 5.04    \\
5051.63  & 0.91   &   $-$2.80  &   5.01     & \nodata  & \nodata  & 5.04    \\
5068.77  & 2.94   &   $-$1.04  &   4.95     & 4.40     & 5.42     & 4.97    \\
5079.74  & 0.99   &   $-$3.22  &   \nodata  & \nodata  & 5.66     & \nodata \\
5083.34  & 0.96   &   $-$2.96  &   4.91     & 4.40     & 5.41     & 4.96    \\
5123.72  & 1.01   &   $-$3.07  &   \nodata  & \nodata  & \nodata  & 5.09    \\
5127.36  & 0.91   &   $-$3.31  &   4.98     & 4.53     & 5.56     & 5.04    \\
5131.47  & 2.22   &   $-$2.52  &   5.01     & 4.53     & 5.65     & 5.10    \\
5141.74  & 2.42   &   $-$2.24  &   4.95     & 4.51     & 5.52     & 5.05    \\
5150.84  & 0.99   &   $-$3.04  &   4.94     & 4.44     & 5.52     & 4.95    \\
5151.91  & 1.01   &   $-$3.32  &   4.95     & 4.54     & 5.66     & 5.06    \\
5166.28  & 0.00   &   $-$4.20  &   4.97     & 4.50     & 5.50     & 5.04    \\
5171.60  & 1.48   &   $-$1.79  &   4.98     & 4.41     & 5.40     & 5.07    \\
5191.45  & 3.04   &   $-$0.55  &   4.94     & 4.35     & 5.62     & 4.94    \\
5192.34  & 3.00   &   $-$0.42  &   4.89     & 4.34     & 5.59     & 4.98    \\
5194.94  & 1.56   &   $-$2.09  &   5.00     & 4.46     & 5.45     & 4.97    \\
5198.71  & 2.22   &   $-$2.14  &   4.89     & 4.44     & 5.52     & 5.04    \\
5216.27  & 1.61   &   $-$2.15  &   4.94     & 4.45     & 5.48     & 5.00    \\
5217.39  & 3.21   &   $-$1.16  &   5.03     & 4.50     & 5.57     & 5.10    \\
5225.53  & 0.11   &   $-$4.79  &   4.98     & 4.52     & 5.54     & 5.08    \\
5232.94  & 2.94   &   $-$0.06  &   4.84     & 4.31     & 5.43     & 4.96    \\
5242.49  & 3.63   &   $-$0.97  &   5.03     & 4.44     & 5.51     & 5.03    \\
5266.56  & 3.00   &   $-$0.38  &   4.91     & 4.33     & 5.51     & 4.94    \\
5281.79  & 3.04   &   $-$0.83  &   4.95     & 4.35     & 5.50     & 4.97    \\
5283.62  & 3.24   &   $-$0.52  &   \nodata  & 4.45     & 5.63     & 5.08    \\
5288.52  & 3.69   &   $-$1.51  &   5.02     & \nodata  & 5.41     & 4.89    \\
5307.36  & 1.61   &   $-$2.99  &   4.92     & 4.41     & 5.50     & 4.99    \\
5322.04  & 2.28   &   $-$2.80  &   4.87     & 4.36     & 5.44     & 4.89    \\
5332.90  & 1.56   &   $-$2.78  &   4.86     & 4.42     & 5.52     & 4.93    \\
5339.93  & 3.27   &   $-$0.72  &   5.00     & 4.49     & 5.62     & 5.08    \\
5364.87  & 4.45   &   $+$0.23  &   5.08     & 4.56     & 5.47     & 5.09    \\
5365.40  & 3.57   &   $-$1.02  &   4.84     & \nodata  & 5.35     & 4.94    \\
5367.47  & 4.42   &   $+$0.44  &   4.92     & 4.42     & 5.46     & 4.93    \\
5369.96  & 4.37   &   $+$0.54  &   4.88     & 4.36     & 5.40     & 4.90    \\
5371.49  & 0.96   &   $-$1.64  &   5.04     & \nodata  & 5.40     & 5.02    \\
5379.57  & 3.69   &   $-$1.51  &   \nodata  & \nodata  & 5.48     & 5.04    \\
5383.37  & 4.31   &   $+$0.64  &   4.83     & 4.34     & \nodata  & \nodata \\
5397.13  & 0.91   &   $-$1.99  &   5.07     & \nodata  & 5.41     & 5.03    \\
5405.77  & 0.99   &   $-$1.84  &   5.03     & \nodata  & 5.39     & 5.05    \\
5410.91  & 4.47   &   $+$0.40  &   4.87     & 4.42     & 5.40     & 4.98    \\
5415.20  & 4.39   &   $+$0.64  &   4.81     & 4.44     & 5.37     & 4.92    \\
5429.70  & 0.96   &   $-$1.88  &   \nodata  & 4.47     & 5.64     & \nodata \\
5434.52  & 1.01   &   $-$2.12  &   5.04     & 4.43     & 5.40     & 5.07    \\
5497.52  & 1.01   &   $-$2.85  &   5.02     & 4.55     & 5.60     & 5.06    \\
5501.47  & 0.96   &   $-$3.05  &   5.03     & 4.56     & 5.58     & 5.13    \\
5506.78  & 0.99   &   $-$2.80  &   5.05     & 4.54     & 5.56     & 5.12    \\
5586.76  & 3.37   &   $-$0.14  &   4.95     & 4.35     & 5.44     & 4.97    \\
5662.52  & 4.18   &   $-$0.57  &   5.02     & 4.54     & 5.63     & \nodata \\
5701.54  & 2.56   &   $-$2.22  &   5.10     & \nodata  & \nodata  & \nodata \\
5753.12  & 4.26   &   $-$0.69  &   \nodata  & 4.43     & 5.59     & \nodata \\
5816.37  & 4.55   &   $-$0.60  &   \nodata  & \nodata  & 5.45     & 4.91    \\
6065.48  & 2.61   &   $-$1.53  &   4.89     & 4.37     & 5.48     & 4.96    \\
6136.61  & 2.45   &   $-$1.40  &   5.02     & 4.48     & 5.56     & 5.08    \\
6137.69  & 2.59   &   $-$1.40  &   4.97     & 4.44     & 5.57     & 5.03    \\
6151.62  & 2.18   &   $-$3.30  &   \nodata  & \nodata  & 5.62     & \nodata \\
6191.56  & 2.43   &   $-$1.42  &   5.03     & \nodata  & 5.47     & 5.02    \\
6213.43  & 2.22   &   $-$2.48  &   5.01     & 4.44     & 5.49     & 5.01    \\
6219.28  & 2.20   &   $-$2.43  &   5.00     & 4.55     & 5.64     & 5.11    \\
6230.72  & 2.56   &   $-$1.28  &   5.04     & 4.53     & 5.64     & 5.13    \\
6240.65  & 2.22   &   $-$3.17  &   \nodata  & 4.33     & 5.49     & \nodata \\
6246.32  & 3.60   &   $-$0.88  &   5.03     & 4.49     & 5.57     & 5.15    \\
6265.13  & 2.18   &   $-$2.55  &   5.04     & \nodata  & 5.58     & 5.12    \\
6297.79  & 2.22   &   $-$2.74  &   \nodata  & 4.44     & 5.44     & \nodata \\
6322.69  & 2.59   &   $-$2.43  &   \nodata  & \nodata  & 5.60     & \nodata \\
6344.15  & 2.43   &   $-$2.92  &   4.88     & 4.49     & 5.55     & \nodata \\
6355.03  & 2.85   &   $-$2.29  &   \nodata  & 4.47     & 5.53     & 5.08    \\
6393.60  & 2.43   &   $-$1.58  &   5.09     & 4.52     & 5.59     & 5.13    \\
6421.35  & 2.28   &   $-$2.03  &   5.04     & 4.51     & 5.61     & 5.10    \\
6430.85  & 2.18   &   $-$2.01  &   5.02     & 4.51     & 5.56     & 5.07    \\
6494.98  & 2.40   &   $-$1.27  &   5.04     & 4.44     & 5.54     & 5.09    \\
6592.91  & 2.73   &   $-$1.47  &   4.92     & 4.42     & 5.51     & 5.07    \\
6593.87  & 2.43   &   $-$2.42  &   5.01     & \nodata  & 5.56     & \nodata \\
6609.11  & 2.56   &   $-$2.69  &   4.86     & 4.38     & 5.49     & 4.96    \\
6677.99  & 2.69   &   $-$1.42  &   5.05     & 4.51     & 5.65     & 5.11    \\
6750.15  & 2.42   &   $-$2.62  &   5.06     & 4.48     & 5.56     & 5.08    \\
\hline\hline
\multicolumn{7}{c}{Fe~\textsc{ii}} \\
\hline
2351.20  & 2.66  &  $-$0.22   &  5.39     & \nodata  & 5.47     & 5.05    \\
2351.67  & 5.25  &  $-$0.05   &  5.04     & \nodata  & \nodata  & \nodata \\
2352.31  & 5.26  &  $+$0.16   &  5.33     & \nodata  & \nodata  & \nodata \\
2372.36  & 2.58  &  $-$2.35   &  5.03     & \nodata  & \nodata  & 4.98    \\
2418.17  & 2.58  &  $-$1.85   &  4.94     & \nodata  & \nodata  & \nodata \\
2422.69  & 3.89  &  $+$0.01   &  5.25     & \nodata  & \nodata  & 5.05    \\
2434.73  & 4.08  &  $+$0.48   &  5.18     & \nodata  & \nodata  & 5.14    \\
2461.28  & 3.23  &  $+$0.23   &  5.32     & \nodata  & \nodata  & 5.26    \\
2463.28  & 3.15  &  $-$0.19   &  5.09     & \nodata  & \nodata  & 5.03    \\
2465.91  & 3.22  &  $-$0.05   &  5.12     & \nodata  & \nodata  & 5.06    \\
2481.05  & 3.24  &  $-$0.79   &  4.87     & \nodata  & \nodata  & \nodata \\
2482.12  & 2.63  &  $-$0.08   &  5.13     & \nodata  & \nodata  & 5.19    \\
2503.33  & 3.15  &  $-$0.08   &  5.00     & \nodata  & \nodata  & 5.03    \\
2503.87  & 3.77  &  $+$0.32   &  4.92     & \nodata  & 5.59     & \nodata \\
2511.76  & 2.69  &  $+$0.34   &  4.97     & \nodata  & \nodata  & 4.96    \\
2542.74  & 3.34  &  $-$0.50   &  4.99     & \nodata  & \nodata  & 4.92    \\
2572.97  & 2.89  &  $-$1.20   &  4.97     & \nodata  & \nodata  & \nodata \\
2620.17  & 2.84  &  $-$1.15   &  5.11     & \nodata  & \nodata  & 5.03    \\
2637.64  & 3.34  &  $-$0.56   &  4.98     & \nodata  & 5.56     & 4.78    \\
2639.56  & 3.34  &  $-$0.78   &  4.94     & \nodata  & 5.54     & 4.77    \\
2657.92  & 3.77  &  $-$1.46   &  5.16     & \nodata  & \nodata  & 5.11    \\
2658.25  & 3.97  &  $-$0.75   &  5.08     & \nodata  & \nodata  & 5.01    \\
2686.11  & 3.23  &  $-$2.21   &  5.15     & \nodata  & 5.57     & 5.20    \\
2716.70  & 0.99  &  $-$3.04   &  5.26     & \nodata  & \nodata  & 5.00    \\
2730.73  & 1.08  &  $-$0.90   &  5.07     & \nodata  & \nodata  & 5.15    \\
2751.12  & 3.20  &  $-$0.88   &  5.17     & \nodata  & \nodata  & 5.02    \\
2753.29  & 3.27  &  $+$0.41   &  4.99     & \nodata  & \nodata  & 4.90    \\
2771.19  & 3.77  &  $-$1.22   &  5.17     & \nodata  & \nodata  & 5.14    \\
2771.56  & 3.23  &  $-$2.06   &  5.38     & \nodata  & \nodata  & \nodata \\
2827.43  & 3.24  &  $-$1.40   &  5.24     & \nodata  & \nodata  & 5.09    \\
2831.56  & 3.20  &  $-$0.26   &  \nodata  & 4.82     & 5.64     & \nodata \\
2839.80  & 5.29  &  $-$0.15   &  5.23     & \nodata  & 5.61     & 5.26    \\
2887.31  & 3.42  &  $-$2.03   &  5.38     & \nodata  & \nodata  & \nodata \\
2895.22  & 3.90  &  $-$0.86   &  5.08     & \nodata  & \nodata  & 5.03    \\
2897.27  & 3.42  &  $-$1.05   &  5.03     & \nodata  & 5.51     & 4.89    \\
2979.35  & 1.10  &  $-$2.07   &  5.19     & \nodata  & 5.60     & 4.87    \\
2985.54  & 1.72  &  $-$0.89   &  5.09     & \nodata  & \nodata  & 5.03    \\
3000.06  & 3.81  &  $-$1.61   &  5.12     & \nodata  & \nodata  & 5.14    \\
3259.05  & 3.90  &  $-$0.97   &  \nodata  & 4.85     & 5.63     & 5.14    \\
3285.41  & 1.08  &  $-$3.84   &  5.19     & \nodata  & 5.59     & \nodata \\
3297.88  & 3.94  &  $-$2.17   &  \nodata  & 5.12     & \nodata  & \nodata \\
3416.02  & 2.28  &  $-$3.03   &  5.37     & 5.04     & \nodata  & 5.27    \\
3425.58  & 1.67  &  $-$3.52   &  5.08     & \nodata  & 5.50     & 4.96    \\
3468.68  & 4.15  &  $-$1.53   &  5.33     & 4.94     & 5.73     & \nodata \\
3487.99  & 1.70  &  $-$3.74   &  5.22     & 4.97     & 5.64     & 5.13    \\
3493.47  & 4.15  &  $-$1.23   &  5.27     & \nodata  & 5.71     & 5.26    \\
3494.67  & 2.28  &  $-$3.11   &  5.35     & 5.02     & \nodata  & \nodata \\
3503.47  & 1.72  &  $-$4.01   &  5.25     & 4.93     & 5.69     & 5.21    \\
3507.40  & 2.34  &  $-$3.52   &  \nodata  & 5.10     & \nodata  & 5.30    \\
3508.20  & 1.72  &  $-$4.06   &  5.26     & \nodata  & 5.75     & 5.22    \\
4178.86  & 2.58  &  $-$2.44   &  5.01     & 4.79     & 5.40     & 5.00    \\
4233.17  & 2.58  &  $-$1.81   &  4.97     & 4.89     & \nodata  & 4.92    \\
4491.40  & 2.86  &  $-$2.64   &  5.00     & 4.82     & 5.48     & 4.92    \\
4515.34  & 2.84  &  $-$2.36   &  4.95     & 4.70     & 5.47     & 4.81    \\
4555.89  & 2.83  &  $-$2.25   &  4.98     & \nodata  & \nodata  & 4.86    \\
4576.34  & 2.84  &  $-$2.92   &  5.09     & 4.80     & 5.52     & 4.96    \\
4583.83  & 2.81  &  $-$1.74   &  \nodata  & 4.81     & 5.55     & 4.82    \\
4620.52  & 2.83  &  $-$3.19   &  \nodata  & 4.75     & 5.44     & 4.91    \\
5197.58  & 3.23  &  $-$2.05   &  5.02     & 4.74     & \nodata  & 4.87    \\
5234.62  & 3.22  &  $-$2.21   &  5.18     & 4.96     & 5.64     & 5.12    \\
5276.00  & 3.20  &  $-$1.90   &  5.08     & 4.78     & 5.63     & 4.97    \\
5414.07  & 3.22  &  $-$3.48   &  \nodata  & 4.92     & 5.38     & \nodata \\
\enddata
\tablecomments{
Wavelength-dependent corrections derived from Fe~\textsc{i} have been
applied to the $\log\epsilon$ entries in this Table.
The uncorrected $\log\epsilon$ values may be obtained by
subtracting the values listed in the final column of Table~\ref{corrtab}.
All $\log(gf)$ values have been adopted from the
critical compilation of \citet{fuhr06}.
 }
\end{deluxetable}

